Coding Schemes Based on Reed-Muller Codes for $(d,\infty)$-RLL Input-Constrained Channels

The paper considers coding schemes derived from Reed-Muller (RM) codes, for transmission over input-constrained memoryless channels. Our focus is on the $(d,\infty)$-runlength limited (RLL) constraint, which mandates that any pair of successive $1$s be separated by at least $d$ $0$s. In our study, we first consider $(d,\infty)$-RLL subcodes of RM codes, taking the coordinates of the RM codes to be in the standard lexicographic ordering. We show, via a simple construction, that RM codes of rate $R$ have linear $(d,\infty)$-RLL subcodes of rate $R\cdot{2^{-\left \lceil \log_2(d+1)\right \rceil}}$. We then show that our construction is essentially rate-optimal, by deriving an upper bound on the rates of linear $(d,\infty)$-RLL subcodes of RM codes of rate $R$. Next, for the special case when $d=1$, we prove the existence of potentially non-linear $(1,\infty)$-RLL subcodes that achieve a rate of $\max\left(0,R-\frac38\right)$. This, for $R > 3/4$, beats the $R/2$ rate obtainable from linear subcodes. We further derive upper bounds on the rates of $(1,\infty)$-RLL subcodes, not necessarily linear, of a certain canonical sequence of RM codes of rate $R$. We then shift our attention to settings where the coordinates of the RM code are not ordered according to the lexicographic ordering, and derive rate upper bounds for linear $(d,\infty)$-RLL subcodes in these cases as well. Finally, we present a new two-stage constrained coding scheme, again using RM codes of rate $R$, which outperforms any linear coding scheme using $(d,\infty)$-RLL subcodes, for values of $R$ close to $1$.

==> BCJR_invar.tex <==
\label{subsec:BCJR_invar}

Given the $Q$-graph, $\mathscr{G}_Q^{(d)}$, for the $(d,\infty)$-RLL input constrained BEC, we call its corresponding $(S,Q)$ graph, $\mathscr{G}_{SQ}^{(d)}$, which is constructed following the description in definition \ref{def:SQ_graph}, with the presentation of channel states given in figure \ref{fig:d_inf_constraint}. 


%We note that our family of $(S,Q)$-graphs  possesses the following interesting property:
%
%\begin{proposition}\label{prop:lp}
%	In the setting of the $(d,\infty)$-RLL input-constrained BEC, for the $(S,Q)$-graphs, $\mathscr{G}_{SQ}^{(d)}$, we have that 
%	\begin{equation*}
%	\max_{\{{P}(x|s,v)\}} P(X=1)\leq \frac{1}{d+1},
%	\end{equation*}
%	where the maximum is taken over all input distributions, $\left({P}(\cdot|s,v): s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ such that the resulting Markov chain on $\mathscr{S}\times \mathscr{V}^{(d)}$ has a unique stationary distribution.
%\end{proposition}
%
%We prove Proposition \ref{prop:lp} by casting the maximization problem as a linear program (LP). We then use the weak duality theorem for LPs (see, for example, \cite{boyd}) to find a feasible point of the corresponding dual LP, the objective value at which serves as an upper bound for our maximization problem. The proof is dealt with in Appendix C.

In this subsection, we construct a BCJR-invariant input distribution, $\left(\left(\tilde{P}(x|s,v):x\in \mathscr{X}\right): (s,v)\in \mathscr{S}\times \mathscr{V}^{(d)}\right)$. In tandem, we will also identify the conditional distribution, $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$, for each $v\in \mathscr{V}^{(d)}$, where $\left(\tilde{\pi}(s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_{SQ}^{(d)}$
%, and $\tilde{\pi}(v) = \sum_{s\in \mathscr{S}}\tilde{\pi}(s,v)$.

%Before we do so, it will be useful to put down some additional notation. Now, for $\mathbf{q}\in \mathscr{V}^{(d)}$, let $(k_1^{\mathbf{q}},k_2^{\mathbf{q}},\ldots,k_{d+1}^{\mathbf{q}})$ denote the runlength sequence of $0$s and $?$s, in $\mathbf{q}$, defined as follows:

%If $\mathbf{q}$ begins with a run of $\ell$ $0$s, for $\ell \geq 1$, then $k_1^{\mathbf{q}} = \ell$; otherwise, $k_1^{\mathbf{q}} = 0$. Further, $k_2^{\mathbf{q}}$ is the length of the run of $?$s after the first run (if any) of $0$s; $k_3^{\mathbf{q}}$ is the length of the (second) run of $0$s after the first run of $?$s, and so on. 

%Note that $k_{2i-1}^{\mathbf{q}}$ records the length of a run of $0$s and $k_{2i}^{\mathbf{q}}$ records the length of a run of $?$s, for $i\geq 1$. Also, $k_{d+1}^{\mathbf{q}}\neq 0$ if, and only if, $\mathbf{q}$ is such that $q_{2i-1}=?$ and $q_{2i}=0$, for $i\geq 1$. Observe that $\sum_{i=1}^{d+1}k_i^{\mathbf{q}} = d$ and $k_i^{\mathbf{q}}\geq 0$, for all $i\in [d+1]$. We shall henceforth omit the superscript $\mathbf{q}$ since it will be apparent from the context.

Since our input distribution %$\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$,
must respect the $(d,\infty)$ input constraint, we need that $\tilde{P}(1|s,v)=0$, for $s\in \{0,1,\ldots,d-1\}$, and we hence need only specify $\tilde{P}(1|d,v)$, for each $v\in \mathscr{V}^{(d)}$, to completely determine the input distribution.

To this end, we first associate with every node $v\in \mathscr{V}^{(d)}$, a probability vector, $\boldsymbol{\theta}_v:=\left(\theta_v(s):s\in \mathscr{S}\right)$, of length $d+1$. 
%The vector $\boldsymbol{\theta}_v$ is a proxy for $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$ for a suitably defined input distribution.

We set $\boldsymbol{\theta}_{Q_i} = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. Further, in compliance with the $(d,\infty)$-RLL input constraint, we set $a_{Q_i}:=\tilde{P}(1|d,Q_i) = 0$, for $i\neq d$. Let us pick $a := \tilde{P}(1|d,Q_d)$, such that $a\leq \frac{1}{d+1}$. The reason for the restriction of $a$ to the interval $[0,\frac{1}{d+1}]$ will be made clear in Lemma \ref{lemma:domain}. 
%We shall, for conciseness of notation, represent $a_{Q_d}$ as $a$.

Now, for $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}^{(d)}_{\text{DB}}$, we define an accompanying vector $\boldsymbol{\beta}=(\beta_{0},\beta_{1},\ldots,\beta_{d-1})$, with\\ $\beta_s := |\{i\in [0:s-1]:w_i=0\}|$. In words, $\beta_s$ is the number of $0$s that appear strictly to the left of position $s$ in the $d$-tuple corresponding to $\mathbf{q}$. We then define $\boldsymbol{\theta}_{\mathbf{q}}$ as follows:

For $0\leq s\leq d-1$,
\begin{equation}\label{eq:theta_even}
{\theta}_{\mathbf{q}}(s) = 
\begin{cases}
0, & \text{ if } w_s=0,\\
\frac{a}{(1-a)^{\beta_s}}, & \text{ if }  w_s=\ ?,
\end{cases}
\end{equation}
and $\theta_{\mathbf{q}}(d) = 1-\sum_{s=0}^{d-1}\theta_{\mathbf{q}}(s)$. It is clear from our definition that $\boldsymbol{\theta}_{Q_d} = \mathbf{e}_{d}^{d}$, where $Q_d = (0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%If $d$ is odd, for $\mathbf{q} \in \mathscr{V}_{\text{DB}}^{(d)}$, we set
%\begin{equation}\label{eq:theta_odd}
%\theta_{\mathbf{q}}(s) = 
%\begin{cases}
%a, \ s\in [0:k_{d+1}-1],\\
%0, \ s\in [k_{d+1}:k_{d+1}+k_d-1],\\
%\frac{a}{(\bar{a})^{k_d}}, \ s\in [k_{d+1}+k_d:\sum\limits_{i\geq {d-1}}k_i -1],\\
%0, \ s\in [\sum\limits_{i\geq {d-1}}k_i:\sum\limits_{i\geq {d-2}}k_i-1],\\
%\quad \vdots\\
%\frac{a}{(\bar{a})^{\sum\limits_{i\geq 3: i\ \text{odd}}k_i}}, \ s\in [\sum\limits_{i\geq {3}}k_i:\sum\limits_{i\geq {2}}k_i],\\
%0, \ s\in [\sum\limits_{i\geq {2}}k_i:d-1],
%\end{cases}
%\end{equation}
%and $\theta_{\mathbf{q}}(d) = 1-\sum_{i=1}^{d-1}\theta_{\mathbf{q}}(i)$.

Finally, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, we let $a_{\mathbf{q}}:= \tilde{P}(1|d,\mathbf{q}) = \frac{a}{\theta_{\mathbf{q}}(d)}$. In order for $a_{\mathbf{q}}$ to be a valid probability, it must lie in $[0,1]$, a sufficient condition for which is provided by Lemma \ref{lemma:domain} below.

\begin{lemma}\label{lemma:domain}
	For $a\in [0,\frac{1}{d+1}]$, $a_{\mathbf{q}}\in [0,1]$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$ .
\end{lemma}

%The proof of this lemma is taken up in  Appendix A.
We refer the reader to \cite{fv} for the proof of the lemma above.
\begin{remark}
%Note that this procedure determines the vector $\left(a_v:v\in \mathscr{V}^{(d)}\right)$, thereby specifying the entire input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$.

Our input distribution is aperiodic for $a<\frac{1}{d+1}$ and $\epsilon\neq 1$, as then there exists a self-loop of positive probability, $\bar{a}\bar{\epsilon}$, from the node $(d,Q_d)$ to itself, in $\mathscr{G}_{SQ}^{(d)}$. The feedback capacity at $\epsilon=1$ is well-known to be $C^{\text{fb}}(1) = 0$, and we safely assume, going forward, that $\epsilon\neq 1$.
\end{remark}

%\begin{figure*}[t]
%	\centering
%	\subfloat[]{\includegraphics[width=0.2\linewidth]{1_inf.png}\label{fig:Q_1}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.4\linewidth]{2_inf.png}\label{fig:Q_2}}
%	\caption{The $Q$-graphs $\mathscr{G}^{(1)}_Q$ and $\mathscr{G}^{(2)}_Q$ are shown above in (a) and (b), respectively. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_1 = 0$, in $\mathscr{G}^{(1)}_Q$, and $Q_2 = (0,0)$, in $\mathscr{G}^{(2)}_Q$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%\end{figure*}
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.5]{2_inf_mod.png}
%	\caption{The $Q$-graph $\mathscr{G}^{(2)}_Q$ is shown above. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_2 = (0,0)$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%	\label{fig:Q_2}
%\end{figure}
%Before we set out to prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR invariant, we shall introduce one other piece of notation. For the function $B_s: \Delta(d)\times \mathscr{Y} \rightarrow \Delta(d)$ defined in equation \eqref{eq:bs}, we define the vector $\mathbf{B}(\mathbf{\theta_v},y)$ to be $\left(B_s(\mathbf{\theta_v},y): s\in \mathscr{S}, s\neq d\right)$, for $v\in \mathscr{V}^{(d)}$. For the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$, we can write down $\mathbf{B}(\mathbf{\theta_v},y)$ explicitly. For $v\in \mathscr{V}_{\text{DB}}^{(d)}$,

Before we prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR-invariant, we note that for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$, the value $B_s(\boldsymbol{\theta}_v,y)$ (see equation \eqref{eq:bs}) can be computed explicitly for the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$. 
%\begin{equation*}
%\mathbf{B}(\mathbf{\theta_v},y) = \begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\frac{\theta_{\mathbf{q}}(1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)}\right], \ y=0,\\
%\left[a_\mathbf{q}\theta_{\mathbf{q}}(d),\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation*}
%
For $0\leq s\leq d-1$, and for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, it holds that
\begin{equation}\label{eq:Bs0}
B_s(\boldsymbol{\theta}_\mathbf{q},y) = 
\begin{cases}
0, & \text{ if } s=0,\ y=0\\
\frac{\theta_{\mathbf{q}}(s-1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)} = \frac{\theta_{\mathbf{q}}(0)}{1-a}, & \text{ if } 1\leq s \leq d-1, \ y=0\\
a_\mathbf{q}\theta_{\mathbf{q}}(d) = a & \text{ if } s=0, \ y=?\\
\theta_{\mathbf{q}}(s-1), & \text{ if } 1\leq s \leq d-1, \ y=?\\
1, & \text{ if } s=0, \ y=1\\
0, & \text{ if } 1\leq s \leq d-1, \ y=1,
\end{cases}
\end{equation}
with $B_d(\boldsymbol{\theta}_\mathbf{q},y) = 1 - \sum_{s=0}^{d-1}B_s(\boldsymbol{\theta}_\mathbf{q},y)$, for $y\in \{0,?,1\}$. Note that the vector $\left(B_s(\boldsymbol{\theta}_\mathbf{q},1): s\in \mathscr{S}\right)$ is equal to $\mathbf{e}_0^{d}$.
%which results in
%\begin{equation}\label{eq:bs_BEC}
%\mathbf{B}(\mathbf{\theta_v},y) = 
%\begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a},\frac{\theta_{\mathbf{q}}(1)}{1-a},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a}\right], \ y=0,\\
%\left[a,\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation}
%since $a_\mathbf{q}\theta_{\mathbf{q}}(d)=a$.

Further, if $v=Q_i$, for some $i\in [0:d-1]$, it holds that
\begin{equation}\label{eq:BsQ}
\left(B_s(\boldsymbol{\theta}_v,y): s\in \mathscr{S}\right) = \mathbf{e}_{i+1}^{d},
\end{equation}
for $y\in \{0,?\}$.
%\begin{equation}\label{eq:bs_BEC_2}
%\mathbf{B}(\mathbf{\theta_v},y) = \mathbf{e}_{i+1}^{d},\ \text{for}\ y\in \{0,?\}.
%\end{equation} 
We now note that the following lemma holds:

\begin{lemma}\label{lemma:bcjr}
	The set of probability vectors $\left(\boldsymbol{\theta}_{v}: v\in \mathscr{V}^{(d)}\right)$ along with the input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ satisfies
	\begin{equation}\label{eq:bs_valid}
	\theta_{v^+}(s^+) = B_{s^+}(\boldsymbol{\theta}_v,y),
	\end{equation}
	for every $(s^+,v,y)\in \mathscr{S}\times \mathscr{V}^{(d)}\times \mathscr{Y}$, where $v^+ = \Phi(v,y)$, with $\Phi:\mathscr{V}^{(d)}\times \mathscr{Y}\rightarrow \mathscr{V}^{(d)}$ is the $Q$-node update function.
\end{lemma}
\begin{proof}
	If $v=Q_i$, for some $i\in [0:d-1]$, then, it follows from equation \eqref{eq:BsQ} that 	
	$\mathbf{e}_{i+1}^{d}=\left(B_s(\boldsymbol{\theta}_{Q_i},y):s\in \mathscr{S}\right)
	$ which, in turn, is equal to  $\boldsymbol{\theta}_{Q_{i+1}}$,	
	for $y\in \{0,?\}$. Equation \eqref{eq:bs_valid} then follows by noting that $\Phi(Q_i,y) = Q_{i+1}$, for $y\in \{0,?\}$.
	
	Now, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, when $y=1$, we see from equation \eqref{eq:Bs0} that	
	$\mathbf{e}_{0}^{d}=\left(B_s(\boldsymbol{\theta}_{v},1):s\in \mathscr{S}\right)$, which is equal to $\boldsymbol{\theta}_{Q_{0}}$.
	Since $\Phi(v,1) = Q_{0}$, it follows that equation \eqref{eq:bs_valid} holds.
	
	Now, let $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}_{\text{DB}}^{(d)}$. Then, since $\Phi(\mathbf{q},0) = (0,w_{0},w_{1},\ldots,w_{d-1}))=:\mathbf{q}_0^+$, and $\Phi(\mathbf{q},?) = (?,w_{0},w_{1},\ldots,w_{d-1})=:\mathbf{q}_?^+$,  we see from equations \eqref{eq:theta_even} and \eqref{eq:Bs0} that $\left(B_s(\boldsymbol{\theta}_\mathbf{q},0):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_0}$ and $\left(B_s(\boldsymbol{\theta}_\mathbf{q},?):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_?}$. Thus, equation \eqref{eq:bs_valid} holds in this case too.	
\end{proof}
We now define the joint distribution, $\theta(s,v):=\theta_v(s)\tilde{\pi}(v)$, where $\left(\tilde{\pi}(v):v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_Q^{(d)}$ induced by $\tilde{P}$. From Lemma \ref{lemma:bcjr} and from the lemma below, we get that $\tilde{P}$ is BCJR-invariant.

\begin{lemma}\label{lemma:stat_dist}
	It holds that $\theta(s,v) = \tilde{\pi}(s,v)$, for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$.
\end{lemma}
\begin{proof}
	Fix an $s^+ \in \mathscr{S}$, and a $v^{+}\in \mathscr{V}^{(d)}$. Now,
	\begin{align*}
	&\sum\limits_{s,v,x,y}\theta(s,v)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}\mathds{1}\{v^+=\Phi(v,y)\}\\
	&= \sum\limits_{v,y}\tilde{\pi}(v)\mathds{1}\{v^+=\Phi(v,y)\}\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\times\\
	&\quad \quad \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \mathds{1}\{s^+=f(x,s)\}\\
	&\stackrel{(a)}{=}\theta_{v^+}(s^+)\sum\limits_{v,y}\tilde{\pi}(v)P(y|v)\mathds{1}\{v^+=\Phi(v,y)\}\\
	&=\theta_{v^+}(s^+)\tilde{\pi}(v^+) = \theta(s^+,v^+),
	\end{align*}
	where (a) follows from Lemma \ref{lemma:bcjr}, since $\theta_{v^+}(s^+)P(y|q)=\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}$. Since this holds for all $(s^+,v^+) \in \mathscr{S}\times \mathscr{Y}$, it follows that $\theta(s^+,v^+) = \tilde{\pi}(s^+,v^+)$.
\end{proof}
The lemma above implies that $\boldsymbol{\theta}_v = \tilde{\pi}(\cdot|v)$, and using Lemma \ref{lemma:bcjr}, we can conclude that $\tilde{P}$ is BCJR-invariant.
\begin{remark}
	It can be shown that for a fixed value of $a$, there is a unique BCJR-invariant input distribution on $\mathscr{G}_{SQ}^{(d)}$. 
	%In particular, this means that for a fixed value of $a$, the probability\\ $P(Y=1|\mathbf{q}) = a\epsilon$, for all $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$.
\end{remark}

==> Proof_UB.tex <==
\label{sec:proof_UB}
\begin{proof}
We shall compute the upper bound expression in theorem \ref{thm:UB} by considering the family of $Q$-graphs, $\mathcal{J}:=\{\hat{\mathscr{G}}_Q^{(d)}: d\in \mathbb{N}\}$, where $\hat{\mathscr{G}}_Q^{(d)}$ is shown in figure \ref{fig:G_hat} for some fixed $d$. Let $\hat{\mathscr{G}}_{SQ}^{(d)}$ denote the $(S,Q)$-graph corresponding to $\hat{\mathscr{G}}_Q^{(d)}$. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{UB_Q.png}
	\caption{The $Q$-graph, $\hat{\mathscr{G}}_Q^{(d)}$. The labels on the edges denote outputs.}
	\label{fig:G_hat}
\end{figure*}

It can be shown that the single closed communicating class in $\hat{\mathscr{G}}_{SQ}^{(d)}$ is precisely the collection $\{(i,\hat{Q}_i): i\in [0:d-1]\}\cup \{(s,\hat{Q}_d):s\in [0:d]\}$ of nodes. Further, since the inputs are constrained, it holds that $P(X=1|S=s,Q=\hat{q}) = 0$, for all $(s,\hat{q}) \neq (d,\hat{Q}_d)$, with $(s,\hat{q})$ in the closed class. Therefore, the matrix of conditional input distributions, $[P(x|s,\hat{q})]$, can be parameterized by a single parameter, $p:=P(X=1|S=d,Q=\hat{Q}_d)$.

A simple computation then reveals that the stationary distribution of nodes in the closed communicating class obey:
\begin{align*}
\pi(s,\hat{Q}_s) &= \frac{p\bar{\epsilon}}{1+dp}, \ s\in [0:d-1],\\
\pi(s,\hat{Q}_d) &= \frac{p\epsilon}{1+dp}, \ s\in [0:d-1], \\
\pi(d,\hat{Q}_d) &= \frac{1}{1+dp}.
\end{align*}
Further, it holds that the conditional probability,

\begin{align*}
P(Y=1|\hat{Q}_d) &= P(Y=1,X=1,S=d|\hat{Q}_d)\\
&=p\bar{\epsilon}\frac{\pi(d,\hat{Q}_d)}{\sum_{s=0}^{d}\pi(s,\hat{Q}_d)}\\
&= \frac{p\bar{\epsilon}}{1+dp\epsilon}.
\end{align*}

Then, by Theorem \ref{thm:UB}, it holds that
\begin{align*}
C_{(d,\infty)}^{\text{fb}} &\leq \sup_{P(x|s,q)\in \Omega} I(X;Y|Q)\\
&= \sup_{P(x|s,q)\in \Omega} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(a)}{=} \max_{p\in [0,1]} \bar{\epsilon}\left(\sum_{s=0}^{d}\pi(s,\hat{Q}_d)\right)h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&= \max_{p\in [0,1]} \frac{\bar{\epsilon}(1+dp\epsilon)}{1+dp}h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&\stackrel{(b)}{=} \max_{\delta \in [0,\frac{1}{1+d\epsilon}]} R(\delta),
\end{align*}
where, in (a), we have used the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$, and (b) follows by changing the variable used in the maximization to $\delta:= \frac{p}{1+dp\epsilon}$.

Now, we note that if $\epsilon^{\star}$ satisfies the equation
\[
(d\epsilon)^{\left(\frac{1}{1-\epsilon}+d\right)} = (1+d\epsilon)^d,
\]
then, the derivative evaluated at $\frac{1}{1+d\epsilon^{\star}}$,  $R^{\prime}\left(\frac{1}{1+d\epsilon^{\star}}\right)$, is equal to $0$. Further, from the proof of Corollaries \ref{coroll} in Appendix B, we observe that $R^{\prime}(\delta)$ is strictly decreasing in $\delta$, for $\delta\in [0,1]$. Hence, it follows that for $\epsilon>\epsilon^{\star}$, the derivative, $R^{\prime}\left(\frac{1}{1+d\epsilon}\right)>0$, with $R^{\prime}(0^+)>0$. 

Therefore, the non-causal capacity, which is a maximum over $[0,1]$ of $R(\delta)$, is strictly larger than the upper bound in Proposition \ref{lemma:UB}, for $\epsilon>\epsilon^{\star}$.
\end{proof}

==> Proof_main.tex <==
\label{sec:proof_thm}

\begin{proof}
For the $(d,\infty)$-RLL input-constrained BEC under the BCJR-invariant input distribution $\tilde{P}$ defined in subsection \ref{subsec:BCJR_invar}, we have that
\begin{align*}
I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(b)}{=} \bar{\epsilon}\sum_{v\in \mathscr{V}^{(d)}}\tilde{\pi}(v)h_b(P(X=1|v)) + h_b(\epsilon)- h_b(\epsilon)\\
&\stackrel{(c)}{=} \bar{\epsilon}\sum_{\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}}\tilde{\pi}(\mathbf{q})h_b(P(X=1|\mathbf{q}))\\
&\stackrel{(d)}{=}\bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
\end{align*}
where (a) follows from the fact that $H(Y|X,Q) = H(Y|X) = h_b(\epsilon)$, and (b) from the fact that $P(Y=?|v) = \epsilon$, for all $v\in \mathscr{V}^{(d)}$, with $P(Y=1|v) = \bar{\epsilon}P(X=1|v)$. We additionally use  the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$. Further, (c) holds since $P(X=1|Q_i) = 0$, for $i\in [0:d-1]$. To obtain the equality (d), note that for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$. Hence, from Lemma \ref{lemma:stat_dist}, it follows that that $P(X=1|\mathbf{q}) = a$.

%Now, since for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$, we get from Lemma \ref{lemma:stat_dist} that $P(X=1|\mathbf{q}) = a$. Hence, it follows that
%
%\begin{equation}\label{eq:I_eval}
%I(X;Y|Q) = \bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
%\end{equation}
Further, it is true that
\begin{align}\label{eq:stat_q}
1 &= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + \sum_{i=0}^{d-1}\tilde{\pi}(Q_i) \notag\\
&= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + d\tilde{\pi}(Q_0) \notag\\
&= (1+da\bar{\epsilon})\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}),
\end{align}
where the penultimate equality holds since $\tilde{\pi}(Q_0) = \tilde{\pi}(Q_i)$, for all $i\in [d-1]$. The last equality follows from the observation that $\tilde{\pi}(Q_0) = \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})P(Y=1|\mathbf{q}) = \bar{\epsilon}a\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})$.

Plugging \eqref{eq:stat_q} back into equation (d), we obtain that $I(X;Y|Q) = \frac{h_b(a)}{da+\frac{1}{1-\epsilon}}$, and taking a maximum over all \\$a\in [0,\frac{1}{d+1}]$, we get the required result.
\end{proof}



==> Q-construction.tex <==
\label{sec:Q_const}
%We shall henceforth consider $\mathscr{S} = \{0,1,\ldots,d\}$ to be the state alphabet, for the $(d,\infty)$-RLL input constrained BEC.
%
%
In this section, we shall construct a family of $Q$-graphs, indexed by $d$, and identify a BCJR-invariant input distribution on the $(S,Q)$-graph corresponding to each $Q$-graph in the family.

\subsection{Construction of Q-graphs}
\input{Q-graph_fly.tex}

\subsection{Construction of a BCJR-invariant input distribution}
\input{BCJR_invar.tex}

==> Q-graph_fly.tex <==
%First, we recall the definition of a De Bruijn graph.
%
%\begin{definition}
%	Given an alphabet $\Sigma = \{w_1,w_2,\ldots,w_m\}$, a $k$-dimensional De Bruijn graph $\mathscr{G}_{\text{DB}}^{(k)} = (\mathscr{V}_{\text{DB}}^{(k)},\mathscr{E}_{\text{DB}}^{(k)},\mathscr{L}_{\text{DB}}^{(k)})$ over $\Sigma$ is a labelled, directed graph with vertex set $\mathscr{V}_{\text{DB}}^{(k)}$, edge set $\mathscr{E}_{\text{DB}}^{(k)}$, and a labelling function $\mathscr{L}_{\text{DB}}^{(k)}: \mathscr{E}_{\text{DB}}^{(k)}\rightarrow \Sigma$. Each vertex $v\in \mathscr{V}$ can be uniquely identified by a $k$-tuple over $\Sigma$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(k)}$ can alternatively be written as $\mathbf{v} = (w_1^v,w_2^v,\ldots,w_k^v)$, where $w^v_i \in \Sigma$, for $i\in [k]$. Note that there are $m^k$ vertices in total.
%	
%	The edge set 	
%	\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(k)} = \lbrace\mathbf{e}:\mathbf{e} = &\left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right),\\
%	& \text{ for some $w_1^i,\ldots,w_k^i,w \in \Sigma$}\rbrace.
%	\end{align*}
%	
%	Further, for any edge \\$\mathbf{e} = \left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right)$, we write \\ $\mathscr{L}(\mathbf{e}) = w$.
%\end{definition}
With each value of $d$ corresponding to the $(d,\infty)$-RLL input-constrained BEC, we associate a $Q$-graph, $\mathscr{G}_{Q}^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, with vertex set $\mathscr{V}^{(d)}$, edge multi-set $\mathscr{E}^{(d)}$, and a labelling function $\mathscr{L}^{(d)}: \mathscr{E}^{(d)}\rightarrow \{0,?,1\}$.

We write $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0, Q_1,\ldots,Q_{d-1}\}$, where each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ is uniquely identified by a $d$-tuple over $\{0,?\}$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ can be written as $\mathbf{q} = (w_{0}^q,w_{1}^q,\ldots,w_{d-1}^q)$, where $w^q_i \in \{0,?\}$, for $i\in \{0,1,\ldots,d-1\}$. In what follows, we suppress the superscript $q$, as it will be clear from the context. Note that there are $2^d$ vertices in $\mathscr{V}_{\text{DB}}^{(d)}$. We denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.\footnote{The subscript ``DB'' indicates that the subgraph $\mathscr{G}_{\text{DB}}^{(d)} = (\mathscr{V}_{\text{DB}}^{(d)},\mathscr{E}_{\text{DB}}^{(d)},\mathscr{L}_{\text{DB}}^{(d)})$, of $\mathscr{G}_{Q}^{(d)}$, is a de Bruijn graph of order $d$, on $\{0,?\}$ symbols.}


We now construct the edge multi-set, $\mathscr{E}^{(d)}$. Firstly, for vertices in $\mathscr{V}_{\text{DB}}^{(d)}$, we define the set $\mathscr{E}_{\text{DB}}^{(d)}$ to consist of all edges $\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right)$, for $(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)}$. 
%\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(d)} = & \lbrace\mathbf{e}:\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right),\\
%	& \ \ \ \ \ \text{ for }(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)} \rbrace.
%\end{align*}
%
Further, for any edge $\mathbf{e} = \bigl((w_{0},w_{1}\ldots,w_{d-1})$, $(w,w_{0},w_{1},\ldots,w_{d-2})\bigr)$, we define the labelling function $\mathscr{L}_{\text{DB}}^{(d)}: \mathscr{E}_{\text{DB}}^{(d)}\rightarrow \{0,?\}$ such that $\mathscr{L}_{\text{DB}}^{(d)}(\mathbf{e}) = w$.

%In this discussion, we shall focus on $d$-dimensional De Bruijn graphs, $\mathscr{G}_{\text{DB}}^{(d)}$, over $\Sigma = \{0,?\}$. By the definition above, this is a graph with $2^d$ vertices, each identified by a unique $d$-tuple consisting of $0,?$ symbols. Let us denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%We construct the $Q$-graph, $\mathscr{G}_Q^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, where $\mathscr{E}^{(d)}$ is now taken to be a multi-set, by first adding $d$ additional vertices, $Q_0,Q_1,\ldots, Q_{d-1}$, to $\mathscr{V}_{\text{DB}}^{(d)}$. Hence, $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0,\ldots,Q_{d-1}\}$.

The edge set, $\mathscr{E}^{(d)}$, is constructed by adding to the set $\mathscr{E}_{\text{DB}}^{(d)}$, the edges $(\mathbf{q},Q_0)$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, and, corresponding to each $Q_i$, $i\in [0:d-1]$, two edges, $\mathbf{e}^{Q_i}_1$ and $\mathbf{e}^{Q_i}_2$, from $Q_i$ to $Q_{i+1}$. %Note that the $Q$-graph, $\mathscr{G}_Q^{(d)}$, has parallel edges. %which are precisely the edges from $Q_i$ to $Q_{i+1}$, for $i\in [0:d-1]$.

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=0.7\textwidth]{3_inf_LB_UB.png}
%	\caption{Plot comparing our lower bound with numerical evaluations of the upper bound from \cite{Graph_based}, for $d=3$.}
%	\label{fig:3_inf_compare}
%\end{figure*}



Finally, the labelling function, $\mathscr{L}^{(d)}:\mathscr{E}^{(d)}\rightarrow \{0,?,1\}$ is defined as:
\begin{equation}\label{eq:label}
\mathscr{L}^{(d)}(\mathbf{e})=
\begin{cases}
\mathscr{L}^{(d)}_{\text{DB}}(\mathbf{e}), & \text{ if } \mathbf{e}\in \mathscr{E}^{(d)}_{\text{DB}},\\
1, & \text{ if } \mathbf{e}=(\mathbf{q},Q_0) \text{ for } \mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}},\\
0 & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_1 \text{ for some } i\in [0:d-1],\\
? & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_2 \text{ for some } i\in [0:d-1].
\end{cases}
\end{equation}

%We note that $\mathscr{G}_Q^{(d)}$ satsifies the properties of a $Q$-graph detailed out in Section \ref{sec:Q-graph}. 
The $Q$-graph, $\mathscr{G}^{(1)}_Q$, is identical to the dynamic programming state diagram under the optimal policy, for the $(1,\infty)$-RLL input-constrained BEC \cite{SabBEC}. The $Q$-graph, $\mathscr{G}^{(2)}_Q$, is shown in Figure \ref{fig:Q_2}.

Our family of $Q$-graphs is then given by $\mathscr{H}:=\{\mathscr{G}^{(d)}_Q: d\in \mathbb{N}\}$, with the $Q$-graph $\mathscr{G}^{({d})}_Q$ being used to derive a lower bound for the $({d},\infty)$-RLL input-constrained BEC.
	
%\begin{remark}
%	The nodes $Q_0, Q_1,\ldots, Q_d$ of $\mathscr{G}^{(d)}_Q$ can be interpreted as follows. Let us define, for a fixed output sequence, $y^t$, the length-$(d+1)$ belief vector $\mathbf{z}_t:=\left(P(S_t=s_t|y^t):s_t\in \mathscr{S}\right)$. Note that the vector,  $\mathbf{z}_t$, which is an element of $\Delta(d)$, is precisely the state vector of the dynamic programming (DP) formulation of the feedback capacity problem \cite{Weiss}. The node $Q_i$ corresponds to the DP state $\mathbf{z}_t = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. This, in turn, has the interpretation that the nodes $Q_0,\ldots, Q_d$ represent the belief vectors when the decoder knows the channel state exactly.
%	
%%	Now, consider a node $\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}$, where $\mathbf{q}\in \{0,1\}^d$. Let $i_1,\ldots,i_k$, for $k\leq d$, denote the positions of the $?$ entries in in $\mathbf{q}$. We then interpret $\mathbf{q}$ as a proxy for the belief vector, $\mathbf{z}_t$, with non-zero entries in only the co-ordinates $d+1,d+1-i_1,\ldots,d+1-i_k$. Note that by our interpretation, $Q_d$, which represents the $d$-tuple $(0,\ldots,0)\in \mathscr{V}^{(d)}_{\text{DB}}$, corresponds to the belief vector $\mathbf{e}_{d+1}^{d+1}$, as described in the previous paragraph.
%\end{remark}




==> achrates.tex <==
\label{sec:achrates}

==> fbcode.tex <==
\label{sec:fbcode}
This section presents a simple feedback coding scheme that achieves the lower bound in Theorem \ref{thm:main}. Our labelling-based coding scheme is similar to the coding schemes in \cite{SabBEC} and \cite{0k}. The main feature of the scheme is a dynamically-changing set of possible messages that is known to both the encoder and the decoder at all times. The objective of the encoder is to communicate a sequence of bits that will enable the decoder to narrow down the set of possible messages to a single message.

Each message $m\in [2^{nR}]$ is mapped uniformly to a point in the unit interval, i.e., the message $m$ is mapped to the point $\frac{m-1}{2^{nR}}$. At each time instant $i$, the unit interval is partitioned into sub-intervals that are labelled by either a `$0$' or a `$1$'. The input $x_i$ to the channel is determined using the label of the sub-interval containing the message. 

The coding scheme proceeds as follows: we first pick positive real numbers $\delta_0,\delta_1,\ldots,\delta_d$ such that $\sum\delta_i\leq 1$. To determine the input bits to be sent, we use a set of $d+2$ labellings, $\mathcal{L}_0,\ldots, \mathcal{L}_d,\hat{\mathcal{L}}$, with the interval $[\sum_{j<i}\delta_j,\sum_{j\leq i}\delta_j)$, in $\mathcal{L}_i$, labelled by a `$1$'. Further, labelling $\hat{\mathcal{L}}$ is such that the entire interval $[0,1)$ is labelled by a `$0$'. Figure \ref{fig:labellings} shows an illustration of the set of labellings.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.6\textwidth]{Labellings_new}
	\caption{The set of labellings, $\mathcal{L}_0,\ldots, \mathcal{L}_d$, used in the coding scheme.}
	\label{fig:labellings}
\end{figure}




\begin{algorithm}[t]
	\caption{Coding Scheme}
	\label{alg}
	\begin{algorithmic}[1]		
		\Procedure{Code}{m}       
		\State Set $\mathcal{M}_0 = [2^{nR}]$ and $Y_{1-d}^{0} = (0,\ldots,0)$.
		\State Set Label = $\mathcal{L}_0$.
		\State Set time index $i = 1$.
		\While{$|\mathcal{M}_{i-1}|>1$}
		\State Transmit $X_i = \Gamma(m,\text{Label})$. \Comment{Encoder}
		\If{none of $Y_{i-d}^{i-1}$ is a $1$}
		\If{$Y_i = 0$}
		\State Set $\mathcal{M}_i = \mathcal{M}_{i-1}^{(0)}$.
		\ElsIf{$Y_i=1$}
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}^{(1)}$. 
		\Else
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}$. 
		\EndIf
		\Else
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}$. 
		\EndIf
		\State Label $\leftarrow$ $G(\text{Label},Y_{i-d+1}^{i})$.
		\State Update $i = i+1$.
		\EndWhile
		\State Output $\hat{m}$, where $\mathcal{M}_{i-1} = \{\hat{m}\}$. \Comment{Decoder}
		\EndProcedure
		
	\end{algorithmic}
\end{algorithm} 
The labelling at any time is a function of the channel outputs upto that time instant and can be recursively computed using the previous labelling and previous $d$ channel outputs. Thus, both the encoder and the decoder can compute the labelling used at all times. Let $L_i$ denote the labelling used at time $i$. We fix $L_0 := \mathcal{L}_0$. Then, $L_{i+1} = G(L_i,Y^{i}_{i-d+1})$, where the function $G$ is defined as follows:

\[G(L_i,Y^{i}_{i-d+1}) =
\begin{cases}
	\hat{\mathcal{L}},\ \text{ if one of $Y_{i-d+1}^{i}$ is a 1},\\
	\mathcal{L}_0,\ \text{if $Y_i=0$},\text{ and none} \text{ of $Y_{i-d+1}^{i}$ is a 1},\\
	\mathcal{L}_{\text{$j+1$ mod$(d+1)$}},\ \text{if $L_i = \mathcal{L}_j$, $Y_{i}=?$ and none} \\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \text{of $Y_{i-d+1}^{i}$ is a 1}.\\
	%\mathcal{L}_0,\ \text{if $L_i = \hat{\mathcal{L}}$ and none of $Y_{i-d}^{i}$ is a 1.} 
\end{cases}
\]

The transitions between the labellings can be represented by the finite state machine (FSM) shown in Figure \ref{fig:QUB}. The labellings in conjunction with the message are used to determine the bit $X_{i+1}$ to be transmitted. Formally, $X_{i+1} = \Gamma(m,L_{i+1})$, where the function $\Gamma$ is defined as:

\[\Gamma(m,L_{i+1}) =
\begin{cases}
	0,\ \text{if $L_{i+1} = \mathcal{L}_j$, for some $j$, and}\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{$\frac{m-1}{2^{nR}} \notin [\sum_{z<j}\delta_z,\sum_{z\leq j}\delta_z)$},\\
	0,\ \text{if $L_{i+1} = \hat{\mathcal{L}}$},\\
	1,\ \text{if $L_{i+1} = \mathcal{L}_j$, for some $j$, and}\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{$\frac{m-1}{2^{nR}} \in [\sum_{z<j}\delta_z,\sum_{z\leq j}\delta_z)$}.
\end{cases}
\]
The chronological order of a single use of the channel at time $i$, for a fixed message $m$, thus is $L_i\rightarrow X_i\rightarrow Y_i$, with $L_{i+1} = G(L_i,Y_{i-d+1}^{i})$.

For a given output sequence $y^i$, we denote by $\mathcal{M}_i$ the set of \emph{possible messages} after time $i$, i.e., $\mathcal{M}_i := \{m\in [2^{nR}]: P(m|y^{i})>0\}$, with $\mathcal{M}_0:=[2^{nR}]$. Note that both the encoder and the decoder can compute the conditional distribution $P(m|y^{i})$ using Bayes' rule. We use the notation $\mathcal{M}_i^{(0)}$ and $\mathcal{M}_i^{(1)}$ to denote the set of messages labelled by a `$0$' and by a `$1$', respectively, in $\mathcal{M}_i$.

A transmission at time $i$ is said to be \emph{successful} if $|\mathcal{M}_i|<|\mathcal{M}_{i-1}|$. Specifically, a successful transmission can occur in one of two scenarios: the first is $y_i = 1$, and the second is where $y_i = 0$ and none of $y_{i-d}^{i-1}$ is a $1$. After a successful transmission, the set of possible messages is calculated and expanded uniformly to the unit interval. It is easy to see that in the first kind of successful transmission, the new set of possible messages, $\mathcal{M}_i$, is equal to $\mathcal{M}_{i-1}^{(1)}$, and in the second kind, $\mathcal{M}_i$ equals $\mathcal{M}_{i-1}^{(0)}$. Figure \ref{fig:succ} shows an illustration of the second of the two kinds of successful transmissions. Figure \ref{fig:eras} depicts the situation when a sequence of erasures is received. In this case, the new set of possible messages, $\mathcal{M}_i$, is equal to $\mathcal{M}_{i-1}$. This transmission procedure continues repeatedly until the set of possible messages contains one message. Additionally, we note that the coding scheme is zero-error, since at the end of the algorithm, the decoder can uniquely decode the transmitted message. The encoding and decoding procedures are described in Algorithm \ref{alg}. 
\begin{figure*}[!t]
	\centering
	
	\includegraphics[width=0.7\textwidth]{Q_graph}
	\caption{Figure shows the finite-state machine (FSM) that represents transitions between the labellings, with the edges labelled by outputs. Note that the state of the FSM can be computed at the encoder using the knowledge of the past $d$ outputs alone. When the encoder is in state $Q_i$, for $i\in \{0,1,\ldots,d\}$, the labelling used is $\mathcal{L}_i$, and when the encoder is in state $\hat{Q}_i$, for $i\in \{0,1,\ldots,d\}$, the labelling used is $\hat{\mathcal{L}}$.}
	\label{fig:QUB}
\end{figure*}

The construction of the labellings ensures that the $(d,\infty)$-RLL input constraint is obeyed. This can be seen from the fact that if ever $Y_i = 1$ for some $i$, it holds that the next $d$ inputs are all set to be $0$s. Further, the staggered manner in which the sub-intervals are labelled by a $1$ in the labellings $\mathcal{L}_0,\ldots,\mathcal{L}_d$ ensures that the input constraint is satisfied when a sequence of erasures is received, too. 

The analysis of the rate of the feedback coding scheme is similar to the proofs of Lemma 3 and Lemma 4 in \cite{0k}. In order to make the exposition self-contained, we repeat parts of the proofs here. For a time index $i\in [n]$, we define $\mathsf{J}_i$ to be the number of information bits gained in a single channel use, which is the logarithm of the change in the size of possible messages at the end of the channel use, i.e.,
\begin{equation}
\label{eq:Jk}
\mathsf{J}_i:= \log_2|\mathcal{M}_{i-1}|-\log_2|\mathcal{M}_{i}|.
\end{equation}
 and $\mathsf{L}_i$ to denote the random variable corresponding to the labelling used, with $\mathsf{L}_i\in \mathcal{L} := \{\hat{\mathcal{L}},\mathcal{L}_0,\ldots,\mathcal{L}_d\}$. The following lemma then holds true:

\begin{lemma}
	\label{lem:gain}
	For any time $i\in [n]$, and for all $\ell\in \mathcal{L}$, we have that $\mathbb{E}[\mathsf{J}_i| \mathsf{L}_i=\ell] = \bar{\epsilon}h_b(\delta_\ell)$, where
	\[\delta_\ell = 
	\begin{cases}
		0,\ \text{if $\ell = \hat{\mathcal{L}}$},\\
		\delta_j,\ \text{if $\ell = \mathcal{L}_j$}.
	\end{cases}
	\]
\end{lemma}
\begin{figure}[!t]
	\centering
	
	\includegraphics[width=0.8\textwidth]{Succ1_2}\label{<figure2>}
	\caption{Figure shows an illustration of a successful transmission of the second kind, when $X_1 = Y_1 = 1$, and when the encoder then transmits $d$ additional zeros. Note that the size of the set of possible messages reduces.}
	\label{fig:succ}
\end{figure}

\begin{figure}[!t]
	\centering
%	\subfloat[]{\includegraphics[width=0.5\linewidth]{Succ1_2}\label{fig:succ}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.5\linewidth]{Eras_4}\label{fig:eras}}
	\includegraphics[width=0.7\textwidth]{Eras_4}
	\caption{The figure shows the setting when two consecutive erasures are received ($Y_1=Y_2=?$), followed by the successful reception of $X_3 = 1$. So long as erasures are received, the set of possible messages is retained as such, while the labellings cycle through $\mathcal{L}_0$ to $\mathcal{L}_d$. Upon the successful reception of $X_3$, the labelling is changed to $\mathcal{L}_0$. However, since the set of possible messages is now a singleton, the transmission ends with the decoder declaring the correct identity of the message.}
	\label{fig:eras}
\end{figure}

\begin{proof}
	We let the random variable $\theta$ denote the indicator that the current output is unerased, i.e.,
	\[
	\theta_i = \mathds{1}\{Y_i\neq `?'\}.
	\]
	Then,
	\begin{align}
		\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell]&=\epsilon\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 0]+\bar{\epsilon}\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 1] \notag\\
		&= \bar{\epsilon}\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 1] \label{eq:lemm},
	\end{align}
where the second equality holds since if an erasure is received, the set of possible messages remains the same.

We now note that in any of the labellings $\mathcal{L}_j$, it holds that the length of the sub-interval labelled by a `$1$' equals $\delta_j$, and equals $0$ in $\hat{\mathcal{L}}$. Hence, if labelling $\ell \in \mathcal{L}$ is employed, the bit transmitted is distributed according to Ber$(\delta_\ell)$ \footnote{We note as in \cite{0k} that since the messages are discrete points in $[0,1)$, the transmitted bit is actually distributed according to Ber$(\delta_\ell -e_i)$, where $e_i$ is a correction factor that is bounded as $0\leq e_i\leq \frac{1}{|\mathcal{M}_{i-1}|}$. We use Algorithm \ref{alg} for encoding, until a time $t$ such that $|\mathcal{M}_t|\leq 2^{\lambda}$, for an absolute constant, $\lambda>0$. A clean-up coding phase can then be employed, after the labelling-based scheme, similar to \cite[Appendix C]{SabBEC}, using which the remaining at most $\lambda$ bits are then transmitted. The rate of the overall two-stage coding scheme can then be computed to equal the rate calculated using the analysis in this paper.}, where $\delta_\ell$ is as defined in the statement of the theorem.

 Assume that the current size of the set of possible messages, $\mathcal{M}$, equals $k$, with the current labelling used being $\ell$. If the current bit transmitted is received successfully, then, the new set of possible messages has size $k\delta_\ell$, if the current input bit is a `$1$', and is equal to $k\bar{\delta}_\ell$, otherwise. Hence, the expected number of bits required to describe the new set of possible messages is $\bar{\delta}_{\ell} k \log_2(\bar{\delta}_{\ell} k)+\delta_\ell k \log_2(\delta_\ell k) = \log_2(k)-h_b(\delta_{\ell})$. Thus, given that $\mathsf{L}=\ell$, following a successful transmission, the decoder gains $h_b(\delta_{\ell})$ bits of information. Substituting into \eqref{eq:lemm}, we get that
\[
\mathbb{E}[\mathsf{J}|\mathsf{L}=\ell] = \bar{\epsilon}h_b(\delta_\ell).
\]
\end{proof}

The following lemma computes the rate of the proposed coding scheme:
\begin{lemma}
	\label{lem:rate}
	For any $\epsilon \in [0,1]$, the proposed coding scheme achieves a rate
	\[
	R = \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta}),
	\]
	where $R(\vec{\delta})$ is as defined in equation \eqref{eq:R}.
\end{lemma}
\begin{proof}
	Fix $0\leq \delta_0,\delta_1,\ldots,\delta_d\leq 1$, with $\sum_{i=0}^{d}\delta_i \leq 1$. The constraint is chosen so as to ensure that the lengths of the intervals used in the labellings in Figure \ref{fig:labellings} are all non-negative. 
	
	Consider the Markov chain induced by the transitions shown in Figure \ref{fig:QUB}, with the transition probabilities $P(Y=?|q) = \epsilon$, for all $q \in \{Q_0,Q_1,\ldots,Q_d,\hat{Q}_0,\hat{Q}_1,\ldots,\hat{Q}_d\}$, and
	\[
	P(Y=1|q) = 
	\begin{cases}
		\bar{\epsilon}\delta_i, \ \text{if $q = Q_i$, for some $i$},\\
		0, \ \text{otherwise}.
	\end{cases}
	\]
	Let $\pi(\ell)$ denote the stationary probability of using labelling $\ell$, which can be calculated using the stationary probabilities of states of the Markov chain on the FSM. Clearly, for $i\in \{0,1,\ldots,d\}$, $\pi(\mathcal{L}_i)$ equals $\pi(Q_i)$, and $\pi(\hat{\mathcal{L}})$ equals $\sum_{j=0}^{d}\pi(\hat{Q}_j)$. The rate of the coding scheme can be computed to be:
	\begin{align*}
		R &= \lim_{n\rightarrow \infty}  \frac{\log_2 |\mathcal{M}_0|}{n}\\
		&\stackrel{(a)}{=} \lim_{n\rightarrow \infty} \frac{1}{n}\sum_{k=1}^{n}\mathbb{E}[\mathsf{J}_k]\\
		&= \lim_{n\rightarrow \infty}  \frac{1}{n} \sum_{k=1}^{n} \sum_{\ell \in \mathcal{L}} P(\mathsf{L}_k = \ell)\mathbb{E}[\mathsf{J}_k|\mathsf{L}_k = \ell]\\
		&\stackrel{(b)}{=} \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell) \lim_{n\rightarrow \infty}  \frac{1}{n} \sum_{k=1}^{n} P(\mathsf{L}_k = \ell)\\
		&\stackrel{(c)}{=} \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell)\pi(\ell)\\
		&= \sum_{i=0}^{d}\bar{\epsilon}h_b(\delta_i)\pi(\mathcal{L}_i)\\
		&\stackrel{(d)}{=} R(\vec{\delta}),
	\end{align*}
where 
\begin{enumerate}[label = (\alph*)]
	\item holds from equation \eqref{eq:Jk},
	\item follows from Lemma \ref{lem:gain} and by exchanging the order of the summations,
	\item follows from the definition of stationary probability and from the fact that the random process $(\mathsf{L}_n:n\in \mathbb{N})$ is a positive recurrent, irreducible, aperiodic Markov chain (this follows from the irreducibility and aperiodicity of the graph in Figure \ref{fig:QUB}), and
	\item holds by an explicit calculation of the stationary probabilities of the Markov process $(\mathsf{L}_n:n\in \mathbb{N})$, which are given by:
	\[
	\pi(\ell)=
	\begin{cases}
		\frac{\epsilon^i}{\sum_{j=0}^{d}\epsilon^j + d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)},\ \ell=\mathcal{L}_i,\\
		\frac{d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)}{\sum_{j=0}^{d}\epsilon^j + d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)},\ \ell=\hat{\mathcal{L}}.
	\end{cases}
	\]
\end{enumerate}
Therefore, maximizing over all allowed parameters $\delta_0,\ldots,\delta_d$, it follows that our coding scheme achieves a rate $R = \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta})$.
\end{proof}

We now provide an upper bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, using Theorem \ref{thm:UB}.
\begin{lemma}
	\label{lem:ub}
	For any $\epsilon \in [0,1]$, the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC is bounded as:
	\[
	C^{\text{fb}}_{(d,\infty)}\leq \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta}).
	\]
\end{lemma}
\begin{proof}
	We simply apply Theorem \ref{thm:UB} to the $Q$-graph that is the FSM in Figure \ref{fig:QUB}. The transition probabilities $P(Y=y|q)$ are the same as those in the proof of Lemma \ref{lem:rate}, for $y\in \{0,?,1\}$ and $q \in \{Q_0,Q_1,\ldots,Q_d,\hat{Q}_0,\hat{Q}_1,\ldots,\hat{Q}_d\}$. Note that the definition of the transition probabilities implies that 
	\[
	P(X=1|q) = 
	\begin{cases}
		\delta_i, \ \text{if $q = Q_i$, for some $i$},\\
		0, \ \text{otherwise}.
	\end{cases}
	\]
	 We then have that
	 \begin{align*}
	 	I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - H(Y|X)\\
	 	&= H(Y|Q) - h_b(\epsilon)\\
	 	&\stackrel{(b)}{=} \bar{\epsilon}H(X|Q)+h_b(\epsilon) - h_b(\epsilon)\\
	 	&= \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell)\pi(\ell)\\
	 	&= \sum_{i=0}^{d}\bar{\epsilon}h_b(\delta_i)\pi(\mathcal{L}_i)\\
	 	&= R(\vec{\delta}),
	 \end{align*}
 where
 \begin{enumerate}[label = (\alph*)]
 	\item holds due to the memorylessness of the BEC, and
 	\item follows from the simple identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$.
 \end{enumerate}
Hence, all that remains to be shown for the proof to be complete is that 
\[
\sup_{\{P(x|s,q)\}} R(\vec{\delta}) = \max_{\sum_{i=0}^{d}\delta_i \leq 1}R(\vec{\delta}).
\]
This is true since for any valid input distribution $\{P(x|s,q)\}$ on the $(S,Q)$-graph corresponding to the $Q$-graph in Figure \ref{fig:QUB}, it holds that
\begin{align*}
	\sum_{i=0}^{d}\delta_i = \sum_{i=0}^{d}P(X=1|Q_i)
	&= \sum_{i=0}^{d}\frac{P(X=1,Q_i)}{\pi(\mathcal{L}_i)}\\
	&{=} \sum_{i=0}^{d}\frac{P(X=1,Q_i)}{\epsilon^i \pi(\mathcal{L}_0)}\\
	&= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,Q_i).	
\end{align*}
Now,
\begin{align*}
    \sum_{i=0}^{d}\delta_i &= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,Q_i)\\
    &= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,S=d,Q_i)\\
    &\leq \frac{1}{ \pi(\mathcal{L}_d)}\left(\sum_{i=0}^{d-1}\epsilon^{d-i}P(X=1,S=d,Q_i)+P(S=d,Q_d)\right)\\
    &= \frac{1}{ \pi(\mathcal{L}_d)}\left(\sum_{i=0}^{d-1}P(S=i,Q_d)+P(S=d,Q_d)\right)\\
    &=1,
\end{align*}
where the penultimate equality holds from the structure of the $(S,Q)$-graph.
\end{proof}
\begin{remark}
	We note that for the case when $d=2$, the authors in \cite{0k} provide the optimal $Q$-graph of Figure \ref{fig:QUB} for evaluating an upper bound on the feedback capacity. We have shown here that their upper bound is tight.
\end{remark}
Lemmas \ref{lem:rate} and \ref{lem:ub}, taken together, prove Theorem \ref{thm:main}. We thus obtain an exact characterization of the feedback capacity, in addition to providing an explicit coding scheme.

==> introduction.tex <==

Discrete memoryless channels (DMCs) were introduced by Shannon \cite{Sh48} as models for communication links, and have, since then, been the object of much research activity in information theory. It was shown by Shannon \cite{Sh56} that causal, noiseless feedback of the outputs does not increase the capacity of memoryless channels, which is given by $C = \sup_{P(x)}I(X;Y)$.


In this paper, we consider DMCs with input constraints, which are specific instances of discrete channels with memory, and which find application in magnetic and optical recording systems \cite{Roth}, \cite{Immink}. Such channels fall under the broad category of finite-state channels (or FSCs), the numerical computation of whose non-feedback capacities has been considered in works such as \cite{GBAA} and \cite{Han3}. Figure \ref{fig:genconstdmc} shows a generic DMC with input constraints, with causal, noiseless feedback. The computation of the feedback capacity of an FSC using a dynamic programming (DP) formulation first appeared in \cite{Chen} and was later extended in works such as \cite{Tatikonda1} and \cite{Tatikonda2}. In this work, we shall focus on the binary erasure channel (or BEC), the inputs of which are constrained to obey the $(d,\infty)$-runlength limited (RLL) input constraint\footnote{The $(d,\infty)$-RLL constraint is a special case of the $(d,k)$-RLL constraint on binary sequences, which requires that the length of any run of consecutive $0$s is at least $d$ and at most $k$.}, which mandates that there needs to be at least $d$ $0$s between any pair of successive $1$s. Such RLL input constraints are necessary for mitigating inter-symbol interference and timing and synchronization errors. As was shown in the works \cite{SabBEC}, \cite{Hanerasure}, and \cite{SabBIBO}, the capacities of the $(1,\infty)$-RLL input-constrained binary erasure and binary symmetric channels are strictly larger than their respective non-feedback capacities, for at least some values of the channel parameters, thereby demonstrating that for channels with memory, feedback may indeed increase capacity.

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.4]{genconstdmc.png}
	\caption{System model of an input-constrained DMC with causal, noiseless feedback.}
	\label{fig:genconstdmc}
\end{figure}

In the context of the BEC with input constraints, the feedback capacities of the $(1,\infty)$- and the $(0,k)$-RLL input constraints (for $k\geq 1$) were computed in the works \cite{SabBEC} and \cite{0k}, respectively. Both of these works put down an explicit coding scheme, whose rate equals the capacity of the BEC with non-causal knowledge of erasures\footnote{Informally, the non-causal capacity is the maximum achievable rate of a coding scheme for the BEC in a setting in which the encoder knows, \emph{prior} to the transmission of the $i^{\text{th}}$ bit $x_i$, whether or not $x_i$ will be erased.}, which, in turn, is as an upper bound on the feedback capacity. Interestingly, this gives rise to the fact that the non-causal capacities of the BEC with the $(1,\infty)$- and the $(0,k)$-RLL input constraints are equal to the respective feedback capacities. Moreover, it was shown in \cite{0k} that the feedback capacity of the $(2,\infty)$-RLL input-constrained BEC is less than the corresponding non-causal capacity, when the channel parameter, $\epsilon$, is equal to $0.5$. In this paper, we show that for the $(2,\infty)$-RLL input-constrained BEC, the feedback capacity is in fact equal to the non-causal capacity for $\epsilon\in [0,1-\frac{1}{2\log(3/2)}]$. This result is a by-product of the main theorem in our paper, which presents an analytical lower bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, for all $d$ greater than or equal to $1$. For the case when $d=1$, our lower bound is tight for all values of $\epsilon$ \cite{SabBEC}, and for $d=2$, our lower bound is numerically close to an upper bound derived using techniques in \cite{Graph_based}, for $\epsilon$ larger than $1-\frac{1}{2\log(3/2)}$, too. We also present analytical upper bounds on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, which, like our lower bounds, are single-parameter optimization problems. We observe that our bounds differ from the non-causal capacity expression (see \cite{0k}) in only the domain of maximization. 

Our techniques involve the use of the single-letter bounding techniques of Sabag et al. in \cite{Single}, and we come up with a specific $Q$-graph (or a $Q$-context mapping) and a choice of a specific ``BCJR-invariant'' input distribution, which gives rise to an achievable rate.

==> perm.tex <==
\label{sec:perm}
Throughout the previous sections, we have assumed that the coordinates of the Reed-Muller code are ordered according to the standard lexicographic ordering. Since permutations of coordinates have the potential to convert a binary word that does not respect the $(d,\infty)$-RLL constraint to one that does, we ask the question if under alternative coordinate orderings, we can obtain linear $(d,\infty)$-RLL subcodes of RM codes, of rate larger than the upper bound in Theorem \ref{thm:rmlinub}.

First, we consider a Gray ordering of coordinates of the code RM$(m,r)$. In such an ordering, consecutive coordinates $\mathbf{b} = (b_1,\ldots,b_m)$ and $\mathbf{b}^\prime = (b_1^\prime,\ldots,b_m^\prime)$ are such that for some bit index $i\in [m]$, $b_i\neq b_i^\prime$, but $b_j = b_j^\prime$, for all $j\neq i$. In words, consecutive coordinates in a Gray ordering, when represented as $m$-tuples, differ in exactly one bit index. Note that multiple orderings are possible, which satisfy this property. We remark that any fixed Gray ordering can also be seen as a Hamiltonian path (see, for example, \cite{diestel}, Chap. 10) on the $m$-dimensional unit hypercube. 

In what follows, we work with a fixed sequence of Gray orderings defined as follows: let $(\pi_m^\text{G})_{m\geq 1}$ be a sequence of permutations, with $\pi_m^\text{G}: [0:2^m-1]\rightarrow [0:2^m-1]$, for any $m\geq 1$, having the property that \textbf{B}$(\pi_m^\text{G}(j))$ differs from \textbf{B}$(\pi_m^\text{G}(j-1))$ in exactly one bit index, for any $j\in [0:2^m-1]$. Here, again, \textbf{B}$(z)$ is the $m$-length binary representation of $z$, for $z\in [0:2^m-1]$. 

Now, fix a sequence of codes $\{{\mathcal{C}_m}(R) = \text{RM}(m,r_m)\}_{m\geq 1}$ that achieves a rate $R\in (0,1)$ over the unconstrained BMS channel, with $r_m\leq m-1$, for all $m$. We again use the notation $K_m:={m\choose \leq r_m}$ to denote the dimension of ${{\mathcal{C}_m(R)}}$. We then define the sequence of Gray-ordered RM codes $\{\mathcal{C}_m^{\text{G}}(R)\}_{m\geq 1}$, with
\begin{align*}\mathcal{C}_{m}^\text{G}(R):= \big\{(c_{\pi_m^\text{G}(0)},c_{\pi_m^\text{G}(1)}&,\ldots,c_{\pi_m^\text{G}(2^m-1)}):\\ &(c_0,c_1,\ldots,c_{2^m-1})\in {\mathcal{C}}_m(R)\big\}.\end{align*}
Clearly, the sequence of codes $\{\mathcal{C}_m^{\text{G}}(R)\}_{m\geq 1}$ also achieves a rate $R\in (0,1)$ over the unconstrained BMS channel. In order to obtain an upper bound on the rate of the largest linear $(d,\infty)$-RLL subcode of the code $\mathcal{C}_m^{\text{G}}(R)$, as in Section \ref{sec:rmublin}, we shall work with the same information set $\mathcal{I}_{m,r_m}$ as in Lemma \ref{lem:infoset}. Note that the coordinates of the Gray-ordered RM code are now represented by $m$-tuples, in which the $j^\text{th}$ coordinate from the beginning is \textbf{B}$(\pi_m^\text{G}(j-1))$.

Again, we define the set
\begin{align*}
\Gamma_{m,r_m}^\text{G}:=\{\pi_m^\text{G}(s):\ &\textbf{B}(\pi_m^\text{G}(s+1))\notin \mathcal{I}_{m,r_m},\ \textbf{B}(\pi_m^\text{G}(s-p)),\ldots,\\&\textbf{B}(\pi_m^\text{G}(s))\in \mathcal{I}_{m,r_m},\text{ for some $p\geq 0$}\},
\end{align*}
to be set of right end-point coordinates of runs that belong to $\mathcal{I}_{m,r_m}$, with the number of such runs being $\left \lvert \Gamma_{m,r_m}^\text{G}\right \rvert$.

We now state and prove a lemma analogous to Lemma \ref{lem:runs}:
\begin{lemma}
	\label{lem:runsgray}
	Under a fixed Gray ordering defined by $\pi_m^\text{G}$, it holds that $\left \lvert\Gamma_{m,r_m}^\text{G} \right \rvert \leq {m\choose r_m+1}$, for $0\leq r_m\leq m-1$.
\end{lemma}
\begin{proof}
	As before, every run of coordinates that belong to $\mathcal{I}_{m,r_m}$ has a right end point, which is an integer $\pi_m^\text{G}(s)\in [0:2^m-2]$, such that wt$(\mathbf{B}(\pi_m^\text{G}(s)))\leq r_m$, but wt$(\mathbf{B}(\pi_m(s+1)))\geq r_m+1$. Now, under the Gray ordering, since consecutive coordinates differ in exactly one bit index, it can be seen that an integer $\pi_m^\text{G}(s) \in \Gamma_{m,r_m}^\text{G}$, only if wt$(\mathbf{B}(\pi_m^\text{G}(s+1)))= r_m+1$. Thus, the number of runs is bounded above by ${m\choose r_m+1}$, which is the number of appearances of coordinates whose binary representation has weight exactly $r_m+1$.
\end{proof}

With Lemma \ref{lem:runsgray} established, we now embark on a proof of Theorem \ref{thm:grayinf}.
\begin{proof}[Proof of Theorem \ref{thm:grayinf}]
	Similar to the proof of Theorem \ref{thm:rmlinub}, the calculation of the overall number, $t_m^\text{G}$, of disjoint $(d+1)$-tuples of consecutive coordinates in $\mathcal{I}_{m,r_m}$, results in
	\begin{align*}
		t_m^\text{G} \geq \frac{K_m}{d+1}-{m\choose r_m+1}.
	\end{align*}
	Again, using Proposition \ref{prop:linub}, it follows that the dimension of any linear $(d,\infty)$-RLL subcode of ${\mathcal{C}_m^\text{G}(R)}$ is at most $K_m-dt_m^\text{G}$. Now, we recall the definition of $\mathsf{R}^{(d,\infty)}_{{\mathcal{C^\text{G}}},\text{Lin}}(R)$, from equation \eqref{eq:Rubgray}. It then holds that $\mathsf{R}^{(d,\infty)}_{{\mathcal{C^\text{G}}},\text{Lin}}(R)$ obeys:
	%It then holds that, under the Gray ordering, the rate, $\mathsf{R}^{(d,\infty)}_{{\mathcal{C^\text{G}}},\text{Lin}}(R)$, of the largest $(d,\infty)$-RLL subcode of ${\mathcal{C}_m^\text{G}(R)}$, obeys
	\begin{align*}
		\mathsf{R}^{(d,\infty)}_{{\mathcal{C^\text{G}}},\text{Lin}}(R)&\leq \limsup_{m\to \infty}\frac{K_m-dt_m^\text{G}}{2^m}\\
		&\leq \limsup_{m\to \infty}\frac{K_m-\frac{dK_m}{d+1}+d\cdot {m\choose r_m+1}}{2^m}\\
		&\leq \lim_{m\to \infty}\frac{\frac{K_m}{d+1}+d\cdot {m\choose \left \lfloor \frac{m}{2}\right \rfloor}}{2^m}\\
		&= \frac{R}{d+1},
	\end{align*}
	where the last equality holds for reasons similar to those in the proof of Theorem \ref{thm:rmlinub}. 
\end{proof}
% We state the above conclusions as a theorem, below, which is a more formal restatement of Theorem \ref{thm:grayinf}:
%\begin{theorem}
%	\label{thm:rmgray}
%	For any sequence of RM codes under a Gray ordering, $\{{\mathcal{C}}_m^\text{G}(R)\}$, with rate$(\mathcal{C}_m^\text{G}(R))\xrightarrow{m\to \infty} R$, it holds that 
%	%the rate of the sequence of the largest linear $(d,\infty)$-RLL subcodes of $\{{\mathcal{C}}_m^\text{G}(R)\}$ obeys
%	\[
%	\mathsf{R}^{(d,\infty)}_{{\mathcal{C}^\text{G},\text{Lin}}}(R) \leq \frac{R}{d+1}.
%	\]
%\end{theorem}

Now, we shift our attention to permuted RM codes $\{\mathcal{C}_m^\pi(R)\}_{m\geq 1}$, defined by the sequence of permutations $(\pi_m)_{m\geq 1}$, with $\pi_m: [0:2^m-1]\to [0:2^m-1]$ (see the discussion preceding Theorem \ref{thm:genperminf} in Section \ref{sec:main}). Also recall the definition of $\overline{\mathcal{C}}_{d,\pi}^{(m)}$ be the largest \emph{linear} $(d,\infty)$-RLL subcode of $\mathcal{C}_m^\pi(R)$.
% As with the Gray ordering, we define the sequence of $\pi$-ordered RM codes $\{\mathcal{C}_m^\pi(R)\}_{m\geq 1}$, with
%\begin{align*}\mathcal{C}_{m}^\pi(R):= \big\{(c_{\pi_m(0)},c_{\pi_m(2)}&,\ldots,c_{\pi_m(N_m-1)}):\\ &(c_0,c_1,\ldots,c_{N_m-1})\in {\mathcal{C}}_m(R)\big\}.\end{align*}
%Note that the sequence of codes $\{\mathcal{C}_m^\pi(R)\}_{m\geq 1}$ also achieves a rate $R$ over the unconstrained BMS channel. We also define $\overline{\mathcal{C}}_{d,\pi}^{(m)}$ be the largest \emph{linear} $(d,\infty)$-RLL subcode of $\mathcal{C}_m^\pi(R)$.
%, and the quantity $\mathsf{R}^{(d,\infty)}_{{\mathcal{C}^\pi},\text{Lin}}(R)$ as follows:

%\begin{equation}
%	\label{eq:Rubgen}
%	\mathsf{R}^{(d,\infty)}_{{\mathcal{C}^\text{G}},\text{Lin}}(R):=\limsup_{m\to \infty}\frac{\log_2\left \lvert \overline{\mathcal{C}}_{d,\text{G}}^{(m)}\right\rvert}{2^m}.
%\end{equation}
We shall now prove Theorem \ref{thm:genperminf}.
\begin{proof}[Proof of Theorem \ref{thm:genperminf}]
	We wish to prove that for ``most'' orderings, and for large $m$, it holds that the rate of $\overline{\mathcal{C}}_{d,\pi}^{(m)}$ is bounded above by $\frac{R}{d+1}+\delta_m$, where $\delta_m \xrightarrow{m\to \infty}0$.
	% where for a sequence of real numbers $(a_m)_{m\geq 1}$ such that $a_m\xrightarrow{m\to \infty} 0$, we write $a_m = o(1)$.
	%$\mathsf{R}^{(d,\infty)}_{{\mathcal{C}^\text{G}},\text{Lin}}(R)\leq \frac{R}{d+1}$. 
	
	To this end, we first make the observation that the sequence of RM codes $\{\mathcal{C}_m(R) = \text{RM}(m,r_m)\}$ achieves a rate $R$ over the BEC, under block-MAP decoding too (see \cite{kud1} and \cite{kud3}). Hence, for large enough $m$, the (linear) RM code $\mathcal{C}_m(R)$ can correct erasures that are caused by a BEC$(1-R-\gamma_m)$, with $\gamma_m>0$, and $\gamma_m\xrightarrow{m\to \infty}0$. This then means that for large $m$, $\mathcal{C}_m(R)$ can correct $2^m(1-R-\gamma_m)-\delta\cdot \sqrt{2^m (1-R-\gamma_m)}$ erasures, with high probability (see Lemma 15 of \cite{abbesw}). Finally, from Corollary 18 of \cite{abbesw}, it then holds that for large enough $m$, any collection of $2^m R(1+\alpha_m)$ columns of $G_\text{Lex}(m,r_m)$, chosen uniformly at random, must have full row rank, $K_m$, with probabilty $1-\delta_m$, with $\alpha_m, \delta_m>0$ and $\alpha_m,\delta_m\xrightarrow{m\to \infty}0$.
	%To this end, we first state the following well-known fact, whose proof we omit, about linear codes that are capacity-achieving over the BEC, under block-MAP decoding. For a sequence of real numbers $(a_n)_{n\geq 1}$ such that $a_n\xrightarrow{n\to \infty} 0$, we write $a_n = o(1)$.
	%\begin{proposition}
	%	\label{prop:blockmap}
	%	For a fixed $R\in (0,1)$, let $\{\mathcal{C}_N(R)\}$ be a sequence of linear codes of increasing blocklength $N$, with dim$(\mathcal{C}_N(R)) =: \kappa_N$. If $\{\mathcal{C}_N(R)\}$ achieves a rate $R$ over the unconstrained BEC, under block-MAP decoding, then for large enough $N$, with probability $1-o(1)$, every collection of $\kappa_N(1+o(1))$ coordinates of $\mathcal{C}_N(R)$ contains an information set.
	%\end{proposition}
	%
	%Now, fix any sequence of RM codes $\{\mathcal{C}_m(R) = \text{RM}(m,r_m)\}$, with rate$(\mathcal{C}_m(R))\xrightarrow{m\to \infty} R$. Pick a large value of $m$ and consider a permutation $\pi_m: [2^m] \to [2^m]$. We define the permuted code $\mathcal{C}_{m}^\pi(R)$ to be such that 
	%\begin{align*}\mathcal{C}_{m}^\pi(R):= \big\{(c_{\pi_m(1)},c_{\pi_m(2)}&,\ldots,c_{\pi_m(N_m)}):\\ &(c_1,c_2,\ldots,c_{N_m})\in {\mathcal{C}}_m(R)\big\}.\end{align*}
	%From \cite{kud1} and \cite{kud3}, we know that the sequence of RM codes $\{\mathcal{C}_m(R) = \text{RM}(m,r_m)\}$ achieves a rate $R$ over the BEC, under block-MAP decoding too. Hence, as a simple corollary of Proposition \ref{prop:blockmap}, we get that for large enough $m$, with probability $1-o(1)$, every $K_m(1+o(1))$ coordinates of $\mathcal{C}_m(R)$ contains an information set, where $K_m={m\choose \leq r_m}$.
	
	In other words, the discussion above implies that for large enough $m$, a collection of $K_m(1+\alpha_m)$ coordinates, chosen uniformly at random, contains an information set, with probabilty $1-\delta_m$. Viewing the above statement differently, it can be argued that for large enough $m$, for a $1-\delta_m$ fraction of the possible permutations $\pi_m: [0:2^m-1]\to [0:2^m-1]$, the first block of $K_m(1+\alpha_m)$ coordinates of the code $\mathcal{C}_{m}^\pi(R)$, contains an information set, ${\mathcal{J}}_{m,r_m}$. Now, within these ``good'' permutations, since $|{\mathcal{J}}_{m,r_m}| = K_m$, it follows that the number of runs, $\left\lvert\Gamma_{m,r_m}^\pi\right \rvert$, of consecutive coordinates that belong to ${\mathcal{J}}_{m,r_m}$, obeys $\left\lvert\Gamma_{m,r_m}^\pi\right \rvert \leq K_m\alpha_m$, with $\Gamma_{m,r_m}^\pi$ defined similar to equation \eqref{eq:gammam}. This is because, the number of runs, $\left\lvert\Gamma_{m,r_m}^\pi\right \rvert$, equals the number of coordinates $s$,  such that $\mathbf{B}(\pi_m(s))\notin {\mathcal{J}}_{m,r_m}$, but $\mathbf{B}(\pi_m(s-1))\in {\mathcal{J}}_{m,r_m}$, and the number of such $s$ is at most $K_m(1+\alpha_m)-K_m$, which equals $K_m\alpha_m$.
	
	Hence, the overall number, $t_m^\pi$, of disjoint $(d+1)$-tuples of consecutive coordinates in $\mathcal{J}_{m,r}$, satisfies (see the proof of Theorem \ref{thm:rmlinub})
	\[
	t_m^\pi\geq \frac{K_m}{d+1}-K_m\alpha_m,
	\]
	for a $1-\delta_m$ fraction of permutations $\pi_m$. Again, applying Proposition \ref{prop:linub}, it holds that for a $1-\delta_m$ fraction of permutations, with $\delta_m\xrightarrow{m\to \infty}0$, the rate of the largest $(d,\infty)$-RLL subcode obeys
	\begin{align*}
		\frac{\log_2\left \lvert \overline{\mathcal{C}}_{d,\text{G}}^{(m)}\right\rvert}{2^m}&\leq \frac{K_m-dt_m^\text{G}}{2^m}\\
		&\leq \frac{K_m-\frac{dK_m}{d+1}+dK_m\alpha_m}{2^m}\\
		&= \frac{R}{d+1}+o(1),
	\end{align*}
	% This implies that the number of disjoint $(d+1)$-tuples of consecutive coordinates in ${\mathcal{J}}_{m,r_m}$ is at least $\left \lfloor \frac{K_m}{d+1} \right \rfloor - K_m\cdot o(1)$. The calculation of $\mathsf{R}^{(d,\infty)}_{{\mathcal{C}^{\pi}},\text{Lin}}(R)$ the proof of Theorem \ref{thm:rmlinub} follows similarly as before, showing that for a $1-o(1)$ fraction of the possible permutations $\pi_m$, it holds that the largest rate of linear $(d,\infty)$-RLL subcodes of $\{\mathcal{C}_m^{\pi_m}\}$ is at most $\frac{R}{d+1}$.
	thereby showing what we set out to prove.
\end{proof}
% We state our findings as a more formal restatement of Theorem \ref{thm:genperminf}:
%\begin{theorem}
%	\label{thm:rmubgen}
%	For large $m$ and for all but an $o(1)$ fraction of coordinate orderings $\pi_m: [0:2^m-1]\to [0:2^m-1]$, the following rate upper bound holds:
%	%it holds that the largest linear $(d,\infty)$-RLL subcode, $\overline{\mathcal{C}}_{d,\pi}^{(m)}$, of the RM code $\mathcal{C}_m^\pi(R)$, obeys the rate upper bound
%		\[
%		\frac{\log_2\left \lvert \overline{\mathcal{C}}_{d,\pi}^{(m)}\right\rvert}{2^m}\leq \frac{R}{d+1}+o(1).
%		\]
%\end{theorem}

==> preamble.tex <==
% preamble.tex

\geometry{letterpaper, top=2.2in, headheight=1.7in}
\date{}

\makeatletter

\def\fulltitle#1{\def\@fulltitle{#1}}
\def\runningtitle#1{\def\@runningtitle{#1}}
\def\runningauthor#1{\def\@runningauthor{#1}}
\def\affiliation#1{\def\@affiliation{#1}}
\def\department#1{\def\@department{#1}}
\def\memoid#1{\def\@memoid{#1}}
\def\theyear#1{\def\@theyear{#1}}
\def\mydate#1{\def\@mydate{#1}}

\runningtitle{How to write an effective report} % Short title
\author{Your name \and John Doe \and Jane Doe} % Full list of authors
\runningauthor{Your name et al.} % Short list of authors
\affiliation{Your University} % Affiliation e.g. University or Company
\department{Your Department} % Department or Office
\memoid{AI Memo 777} % ID of the tech report
\theyear{2018} % year of the tech report
\mydate{August 08, 2018} %the date

\def\displaymydate{\@mydate}
\def\displaytheyear{\@theyear}
\def\displaymemoid{\@memoid}
\def\displaydepartment{\@department}
\def\displayaffiliation{\@affiliation}
\def\displayrunningauthor{\@runningauthor}
\def\displayrunningtitle{\@runningtitle}

\makeatother

\makeatletter
\patchcmd{\@zfancyhead}{\fancy@reset}{\f@nch@reset}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyorh}{\f@nch@orh}{}{}
\makeatother

% ----------
% fancyhdr setup
% ----------

\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}

\fancypagestyle{firstpage}
{
    \fancyhf{}
    \fancyhead{%
        \begin{center}
            \textsc{\displayaffiliation}\\
            \textsc{\displaydepartment}
        \end{center}
        \vspace*{0.5in}
        \displaymemoid
        \hfill
        \displaymydate
    }
    \fancyfoot[L]{\footnotesize \textbf{\textsc{\displayaffiliation} -- \displaytheyear}}
}
\fancyhead[EL]{\small \displayrunningauthor}
\fancyhead[ER]{\small Page \thepage}
\fancyhead[OL]{\small Page \thepage}
\fancyhead[OR]{\small \displayrunningtitle}

\chead{}
\lfoot{}
\cfoot{}
\rfoot{}

% ----------

\providecommand{\keywords}[1]{\noindent \textbf{Keywords:} #1} % keywords definition

\renewcommand{\familydefault}{\sfdefault} % sans-serif font
\setlength{\parskip}{1em} % 1em skip between paragraphs
\abslabeldelim{:} % use colon after the run-in 'Abstract' word
\setlength{\parindent}{0pt} % no indentantion for first page 
\setlength{\abstitleskip}{-\absparindent} % this is because the abstract package sets \absparindent to \parindent

\pretitle{\Large \begin{center}}
\posttitle{\\[2ex] \Large \textbf{by}\end{center}}

==> report_header.tex <==
\usepackage{ifthen}
\usepackage{cite}
\usepackage{algorithm}
\usepackage[cmex10]{amsmath} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)
\usepackage{amsthm,amsfonts,amssymb}
\usepackage[noend]{algpseudocode}
\setcounter{MaxMatrixCols}{17}

\usepackage{subfig}
\usepackage{blkarray}
\usepackage[mathscr]{euscript}
\usepackage{enumitem}
%\usepackage{romannum}
\usepackage{blkarray}
\usepackage{stfloats}%
%\newtheorem{theorem}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}[section]{Lemma}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
%\theoremstyle{definition}
%\newthorem{definition}{Definition}[section]
%\usetikzlibrary{graphs}
\usepackage{url}
\usepackage{arydshln}
\usepackage{mathtools}
\usepackage{dsfont}
%\usepackage{kbordermatrix}
%\newcommand{\indicator}[1]{\mathbb{1}_{\set{#1}}}
%\usepackage{braket}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)

\usepackage{geometry}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[runin]{abstract}
\usepackage{titling}
\usepackage{booktabs}
\usepackage{fancyhdr}
\usepackage{helvet}
\usepackage{csquotes}
\usepackage{graphicx}
\usepackage{blindtext}
\usepackage{parskip}
\usepackage{etoolbox}


==> statphy.tex <==
\label{sec:statphy}
\subsection{Factor Graphs, the BP Algorithm, and the BP Approximation}
In this section, we discuss a technique, based on tools from statistical physics, which can be used to compute estimates of the rate of $(1,\infty)$-RLL subcodes of RM codes. We begin with a short background on factor graphs and some techniques from statistical physics. For a comprehensive treatment of the topic, we refer the reader to \cite{kschischang, gdl, forney} and  \cite{mm}.

Consider a non-negative function $F:\{0,1\}^n\to [0,\infty)$, in $n$ binary variables, $x_1,x_2,\ldots,x_n$. We shall use the vector $\mathbf{x}$ to denote $(x_1,\ldots,x_n)$. Suppose that $F$ enjoys a factorization of the form:
\[
F(x_1,\ldots,x_n) = \prod_{a\in \mathcal{F}} f_a(x_{\partial a}),
\]
where $\mathcal{F}$ is the set of \emph{factors}, indexed by letters of the alphabet, and a given factor $f_a$ acts on the set of variables $x_{\partial a} \subseteq \{x_1,\ldots,x_n\}$. We assume that each factor $f_a$, $a\in \mathcal{F}$, is a non-negative function. We then call $F$ a \emph{product-form function}.

Further, we define the \emph{partition function} of $F$ as
\[
Z := \sum_{\mathbf{x}} F(\mathbf{x}) = \sum_{\mathbf{x}} \prod_{a\in \mathcal{F}} f_a(x_{\partial a}).
\]
It is well-known that in order to calculate $Z$ in a computationally efficient manner, one has to make use of the structure of the factorization of $F$. The most common tool used to represent this structure is the \emph{factor-graph} representation of $F$.

\begin{definition}[see, for example, \cite{kschischang}]
	A factor graph representing $F$ is a bipartite graph that has a variable node for every variable $x_i$, $i\in [n]$, and a factor node for every factor $f_a$, $a\in \mathcal{F}$. Further, an edge connects variable node $x_i$ to factor node $f_a$ if and only if $x_i \in x_{\partial a}$. 
\end{definition} 

\begin{example}
	Consider the linear code $\mathcal{C}$, defined by the parity-check matrix
	\begin{equation}
		\label{eq:tanner}
	H = \begin{bmatrix}
		1 & 1& 0 & 0 & 0\\
		0 & 1 & 1 & 1 & 0\\
		0 & 0 & 0 & 1 &1
	\end{bmatrix}.
	\end{equation}
	Let $\mathbf{h}_i$, $i=1,2,3$, denote the rows of $H$. We define the product-form function $F:= \mathds{1}\{\mathbf{x}\in \mathcal{C}\} = \prod_{i=1}^{3} \mathds{1}\{\mathbf{h}_i \mathbf{x}^T = {0}\}$. Clearly, $F$ can be represented by the factor graph shown in Figure \ref{fig:factor}. The factor graph representing the membership function of a linear code $\mathcal{C}$ is called the Tanner graph (see \cite{tanner, wiberg1}) of $\mathcal{C}$. In this example, the factor graph is a tree.
\end{example}

\begin{figure}[!t]
	\centering
	\resizebox{0.2\textwidth}{!}{
		


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,514); %set diagram left start at 0, and has height of 514
	
	%Shape: Circle [id:dp8456012612079831] 
	\draw   (245.22,173.28) .. controls (245.22,165.27) and (251.71,158.78) .. (259.72,158.78) .. controls (267.73,158.78) and (274.22,165.27) .. (274.22,173.28) .. controls (274.22,181.29) and (267.73,187.78) .. (259.72,187.78) .. controls (251.71,187.78) and (245.22,181.29) .. (245.22,173.28) -- cycle ;
	%Shape: Circle [id:dp480278019589671] 
	\draw   (245.22,223.28) .. controls (245.22,215.27) and (251.71,208.78) .. (259.72,208.78) .. controls (267.73,208.78) and (274.22,215.27) .. (274.22,223.28) .. controls (274.22,231.29) and (267.73,237.78) .. (259.72,237.78) .. controls (251.71,237.78) and (245.22,231.29) .. (245.22,223.28) -- cycle ;
	%Shape: Circle [id:dp7229988381805893] 
	\draw   (245.22,273.28) .. controls (245.22,265.27) and (251.71,258.78) .. (259.72,258.78) .. controls (267.73,258.78) and (274.22,265.27) .. (274.22,273.28) .. controls (274.22,281.29) and (267.73,287.78) .. (259.72,287.78) .. controls (251.71,287.78) and (245.22,281.29) .. (245.22,273.28) -- cycle ;
	%Shape: Circle [id:dp6987188972261212] 
	\draw   (245.22,323.28) .. controls (245.22,315.27) and (251.71,308.78) .. (259.72,308.78) .. controls (267.73,308.78) and (274.22,315.27) .. (274.22,323.28) .. controls (274.22,331.29) and (267.73,337.78) .. (259.72,337.78) .. controls (251.71,337.78) and (245.22,331.29) .. (245.22,323.28) -- cycle ;
	%Shape: Circle [id:dp6258306233683656] 
	\draw   (245.22,373.28) .. controls (245.22,365.27) and (251.71,358.78) .. (259.72,358.78) .. controls (267.73,358.78) and (274.22,365.27) .. (274.22,373.28) .. controls (274.22,381.29) and (267.73,387.78) .. (259.72,387.78) .. controls (251.71,387.78) and (245.22,381.29) .. (245.22,373.28) -- cycle ;
	%Shape: Rectangle [id:dp33706725338569976] 
	\draw   (357,207.78) -- (380,207.78) -- (380,230.52) -- (357,230.52) -- cycle ;
	%Shape: Rectangle [id:dp010116561228115661] 
	\draw   (357,257.91) -- (380,257.91) -- (380,280.65) -- (357,280.65) -- cycle ;
	%Shape: Rectangle [id:dp8735982757105988] 
	\draw   (357,308.04) -- (380,308.04) -- (380,330.78) -- (357,330.78) -- cycle ;
	%Straight Lines [id:da5555789087529314] 
	\draw    (274.22,173.28) -- (357,219.78) ;
	%Straight Lines [id:da9552407466015203] 
	\draw    (274.22,223.28) -- (357,219.78) ;
	%Straight Lines [id:da8819702293734363] 
	\draw    (274.22,223.28) -- (357,269.78) ;
	%Straight Lines [id:da14836423900940343] 
	\draw    (274.22,273.28) -- (357,269.78) ;
	%Straight Lines [id:da41965544130687393] 
	\draw    (274.22,323.28) -- (357,269.78) ;
	%Straight Lines [id:da5519140149646575] 
	\draw    (274.22,323.28) -- (356,319.78) ;
	%Straight Lines [id:da38808679818860214] 
	\draw    (274.22,373.28) -- (356,319.78) ;
	
	% Text Node
	\draw (362,214.18) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{a}$};
	% Text Node
	\draw (362,265.18) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{b}$};
	% Text Node
	\draw (362,315.18) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{c}$};
	% Text Node
	\draw (253,168.7) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 47; blue, 102 }  ,opacity=1 ]  {$x_{1}$};
	% Text Node
	\draw (253,218.7) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 51; blue, 117 }  ,opacity=1 ]  {$x_{2}$};
	% Text Node
	\draw (253,268.7) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 54; blue, 117 }  ,opacity=1 ]  {$x_{3}$};
	% Text Node
	\draw (253,318.7) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 3; green, 43; blue, 94 }  ,opacity=1 ]  {$x_{4}$};
	% Text Node
	\draw (253,368.7) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 3; green, 42; blue, 88 }  ,opacity=1 ]  {$x_{5}$};
	
	
\end{tikzpicture}
}
\caption{Factor graph representing the product-form function $F:= \mathds{1}\{\mathbf{x}\in \mathcal{C}\}$, where $\mathcal{C}$ is defined by the parity-check matrix in \eqref{eq:tanner}. The factors are $f_a(x_1,x_2) = \mathds{1}\{x_1+x_2 =0\ (\text{mod }2)\}$, $f_b(x_2,x_3,x_4) = \mathds{1}\{x_2+x_3 +x_4=0\ (\text{mod }2)\}$, and $f_c(x_4,x_5) = \mathds{1}\{x_4+x_5 =0\ (\text{mod }2)\}$.}
\label{fig:factor}
\end{figure}		


Now, for the special case where the factor graph corresponding to the product-from function $F$ is a tree, the exact computation of $Z$ proceeds via the Sum-Product Algorithm (SPA) \cite{kschischang} (or, in a more general form, the generalized distributive law (GDL) \cite{gdl}). As part of the algorithm, variable and factor nodes pass \emph{messages} to one another, until the messages converge to a fixed value. In particular, at iteration $t\in \{0,1,2,\ldots\}$, given an edge $(x_i,f_a)$ of the factor graph, let $\left(\nu_{i\to a}^{(t)}(x_i): x_i\in \{0,1\}\right)$ be the messages from variable node $x_i$ to factor node $f_a$, and let $\left(\hat{\nu}_{a\to i}^{(t)}(x_i):\ x_i\in \{0,1\}\right)$ be the messages from factor node $f_a$ to variable node $x_i$. The SPA updates then are:
\begin{align}
	\hat{\nu}_{a\to i}^{(t)}(x_i) &= \sum_{x_{\partial a}\setminus x_i} f_a(x_{\partial a}) \prod_{j\in \partial a \setminus \{i\}} \nu_{j\to a}^{(t)}(x_j) \tag{FP1}\\
	\nu_{i\to a}^{(t+1)} (x_i)&= \prod_{b\in \partial i \setminus \{a\}} \hat{\nu}_{b\to i}^{(t)}(x_i), \tag{FP2}
\end{align}
for some initialization of $\left(\nu_{i\to a}^{(0)}(x_i): x_i\in \{0,1\}\right)$, with $\partial a \subseteq [n]$ and $\partial i \subseteq \mathcal{F}$ denoting the neighbours of $f_a$ and $x_i$, respectively, in the factor graph. We shall sometimes call the SPA updates as belief-propagation (BP) updates, after their similarities with Pearl's BP algorithm \cite{pearl}. The partition function is then computed as $Z = \sum_{x_i} \prod_{b\in \partial i} \hat{\nu}_{b\to i}^{\star}(x_i)$, where $\left(\hat{\nu}_{a\to i}^{\star}(x_i): x_i\in \{0,1\}\right)$ and $\left({\nu}_{i\to a}^{\star}(x_i): x_i\in \{0,1\}\right)$ are the fixed-point messages, satisfying (FP1) and (FP2), obtained after convergence of the BP algorithm.

For product-form functions $F$ such that the associated factor graph has cycles, however, it is in general not possible to exactly compute $Z$ as above, but one can obtain estimates of the partition function. A common such estimate is the so-called \emph{Bethe approximation}, $Z^{\text{Bethe}}$ of the partition function (see \cite{yfw} for the definition of the Bethe approximation and \cite{vontobel1,vontobel2,vontobel3} for example computations). We direct the reader to references \cite{ruozzi1} and \cite{ruozzi2} for instances where the Bethe approximation is a lower bound on the actual partition function. In this work, we are interested in the BP approximation, $Z^{\text{BP}}$, which is computed using the fixed-point messages of the BP algorithm, run on the factor graph with cycles, and which is a lower bound on $Z^{\text{Bethe}}$. The BP approximation, $Z^{\text{BP}}$, obeys (see Chapter 14 in \cite{mm})
\begin{equation}
	\label{eq:zbpstart}
	\log_2 Z^{\text{BP}} = \sum_{a\in \mathcal{F}}\log_2 Z_a + \sum_{i\in [n]} \log_2 Z_i - \sum_{\text{edges }(x_i,f_a)} \log_2 Z_{ia},
\end{equation}
where
\begin{align}
	Z_i &= \sum_{x_i} \prod_{a\in \partial i} \hat{\nu}^{\star}_{a\to i}(x_i),\\
	Z_a &= \sum_{x_{\partial a}} f_a(x_{\partial a}) \prod_{i\in \partial a} \nu^{\star}_{i\to a}(x_i),\\
	Z_{ia} &= \sum_{x_i} \nu^{\star}_{i\to a}(x_i) \hat{\nu}^{\star}_{a\to i}(x_i). \label{eq:zbpend}
\end{align}
\subsection{Computing Estimates of Rates of $(1,\infty)$-RLL Subcodes }
In what follows, we shall first establish the relationship between counting the number of $(1,\infty)$-RLL constrained codewords in a Reed-Muller code and the computation of a certain expected log-partition function. We shall then evaluate the BP approximation to the partition function, using insights about the fixed-point messages of the BP updates from (FP1) and (FP2), and hence obtain a lower bound on the Bethe approximation. Finally, we shall point to ways, from the literature, to compare the actual partition function with the Bethe approximation.

Now, fix a sequence of RM codes $\left\{\hat{\mathcal{C}}_m(R) = \text{RM}(m,r_m)\right\}_{m\geq 1}$ such that rate$\left(\hat{\mathcal{C}}_m(R)\right) \xrightarrow{m\to \infty} R$, for $R\in (0,1)$. We shall index coordinates of the codewords in $\hat{\mathcal{C}}_m(R)$ by binary $m$-tuples in the lexicographic order. Recall that under the lexicographic ordering, a codeword Eval$(f) \in \hat{\mathcal{C}}_m(R)$ is $(1,\infty)$-RLL constrained if and only if $g,h$, such that $f=g+x_m\cdot h$, satisfy conditions (C1) and (C2), simultaneously, where
\begin{align*}
	&\text{(C1):  supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$}\\
	&\text{(C2): $h(\boldsymbol{b}) = 0$, if $\boldsymbol{b}\in \Gamma(g)$}.
\end{align*}
Recall the definition
\[
\Gamma(g):= \{\boldsymbol{b} = (b_1,\ldots,b_{m-1}):\ \boldsymbol{b} \text{ is the end of a run of $0$s in Eval$(g)$,} \text{ $\boldsymbol{b}\neq (1,1,\ldots,1)$}\}.
\]
For ease of reading, we use the notation $\mathbf{g}$ and $\mathbf{h}$ for the vectors Eval$(g)$ and Eval$(h)$, respectively. Also, let $\tilde{\mathbf{g}}$ be the $2^{m-1}$-length vector such that $\tilde{g}_\mathbf{b} = 1$, if $\mathbf{b} = (b_1,\ldots,b{m-1})\in \Gamma(g)$, and  $\tilde{g}_\mathbf{b} = g_\mathbf{b} = g(\mathbf{b})$, otherwise. Also, for a fixed $\mathbf{g}$, and a given $\mathbf{h}$, we denote by $\tilde{\mathbf{h}}$ the $2^{m-1}$-length vector with $\tilde{h}_\mathbf{b} = 1+h_{\mathbf{b}}\ (\text{mod } 2)$, if $\mathbf{b} \in \Gamma(g)$, and $\tilde{h}_\mathbf{b} = h_\mathbf{b} = h(\mathbf{b})$, otherwise.

The above definitions lead us to the following equivalent statement of Proposition \ref{lem:necesscond}:

\begin{proposition}
	For Eval$(f)\in \hat{\mathcal{C}}_m(R)$, it holds that Eval$(f) \in S_{(1,\infty)}$ if and only if wt$(\tilde{\mathbf{g}}) = \tilde{\mathbf{g}}\cdot \tilde{\mathbf{h}}$, where $\mathbf{u}\cdot \mathbf{v}$ denotes the inner product (over $\mathbb{F}_2$) between vectors $\mathbf{u}, \mathbf{v} \in \mathbb{F}_2^t$.
\end{proposition}

Now, we define $H_g(h):= \text{wt}(\tilde{\mathbf{g}}) - \tilde{\mathbf{g}}\cdot \tilde{\mathbf{h}}$ to be the \emph{Hamiltonian}, or energy function, at $h$, for a fixed $g$. Note that $H_g(h) = 0$ if and only if $\text{Eval}(f)\in S_{(1,\infty)}$, and $H_g(h)>0$, otherwise. For a fixed \emph{inverse temperature} parameter $\beta>0$, we let
\[
Z_g^{(m)}(\beta):= \sum_h e^{-\beta H_g(h)}\cdot\mathds{1}\{\mathbf{h}\in \mathcal{C}_m^{(h)}\},
\]
where we let $\mathcal{C}_m^{(h)}$, as before, denote $\text{RM}(m-1,r_m-1)$, and $\mathcal{C}_m^{(g)}$ denote $\text{RM}(m-1,r_m)$.
Observe that $$\lim_{\beta \to \infty} Z_g^{(m)}(\beta) = \#\left\{h: \text{deg}(h)\leq r_m-1\text{ and Eval}(g+x_m\cdot h)\in S_{(1,\infty)}\right\},$$ for a fixed $g$. The quantity of interest to us is $Z^{(m)}(\beta):=\sum_g Z_g^{(m)}(\beta)\cdot\mathds{1}\{\mathbf{g}\in \mathcal{C}_m^{(g)}\}$, with the property that 
\begin{equation}
	\label{eq:statphy1}
	\lim_{\beta \to \infty} Z^{(m)}(\beta) = \#\left\{(g,h): \text{Eval}(f)\in S_{(1,\infty)},\text{ where Eval$(f) = \text{Eval}(g+x_m\cdot h)\in \hat{\mathcal{C}}_m(R)$}\right\}.
\end{equation}
\begin{remark}
	The set $\left\{(g,h): \text{Eval}(g+x_m\cdot h)\in S_{(1,\infty)}\text{ and Eval$(g+x_m\cdot h) \in \hat{\mathcal{C}}_m(R)$}\right\}$ is the set of \emph{ground states} (or lowest energy states) of the product-form function $F(g,h) = e^{-\beta H_g(h)}\cdot \mathds{1}\{\mathbf{g}\in \mathcal{C}_m^{(g)}\text{ and } \mathbf{h}\in \mathcal{C}_m^{(h)}\}$, and $Z^{(m)}(\beta)$ is the partition function of $F$.
\end{remark}
From equation \eqref{eq:statphy1}, we get that the rate of $(1,\infty)$-RLL subcodes of $\left\{\hat{\mathcal{C}}_m(R)\right\}_{m\geq 1}$ is
\begin{equation}
	\label{eq:statphy2}
	\mathsf{R}^{(1,\infty)}_{\hat{\mathcal{C}}}(R) = \limsup_{m\to \infty} \lim_{\beta\to \infty} \frac{\log_2 Z^{(m)}(\beta)}{2^m}.
\end{equation}
Now,
\begin{align}
	\mathsf{R}^{(1,\infty)}_{\hat{\mathcal{C}}}(R) &=\limsup_{m\to \infty} \lim_{\beta \to\infty} \frac{1}{2^m}\cdot \log_2\left(\mathbb{E}_{\mathbf{g}\sim \text{Unif}\left(\hat{\mathcal{C}}_m^{g}\right)}\left[Z_g^{(m)}(\beta)\right]\cdot \left\lvert \hat{\mathcal{C}}_m(R)\right\rvert \right) \notag\\
	&= \limsup_{m\to \infty} \lim_{\beta \to\infty} \frac{\log_2\left(\mathbb{E}_{\mathbf{g}\sim \text{Unif}\left(\hat{\mathcal{C}}_m^{g}\right)}\left[Z_g^{(m)}(\beta)\right]\right)}{2^m} + \frac{R}{2} \notag\\
	&{\geq} \limsup_{m\to \infty} \lim_{\beta \to \infty} \frac{\mathbb{E}_{\mathbf{g}\sim \text{Unif}\left(\hat{\mathcal{C}}_m^{g}\right)}\left[\log_2 Z_g^{(m)}(\beta)\right]}{2^m}+\frac{R}{2}, \label{eq:statphy2}
\end{align}
where inequality \eqref{eq:statphy2} holds by an application of Jensen's inequality. Since the exact computation of $Z_g^{(m)}(\beta)$ is difficult, we resort to the computation of the BP approximation, ${Z}_g^{\text{BP}}(\beta)$. For the calculation of ${Z}_g^{\text{BP}}(\beta)$, we need to first construct the factor graph, the product-form function on which has ${Z}_g^{\text{BP}}(\beta)$ as the partition function. To ease matters, we shall first compute
\begin{equation}
	\hat{Z}_g^{\text{BP}}(\beta):= \sum_h e^{+\beta\cdot \tilde{\mathbf{g}}\cdot \tilde{\mathbf{h}}}\cdot\mathds{1}\{\mathbf{h}\in \mathcal{C}_m^{(h)}\},
\end{equation}
for large $m$ and large $\beta>0$, with ${Z}_g^{\text{BP}}(\beta) = e^{-\beta \text{wt}(\tilde{\mathbf{g}})}\cdot \hat{Z}_g^{\text{BP}}(\beta)\cdot \mathds{1}\{\mathbf{g}\in \mathcal{C}_m^{(g)}\}$. To do so, we run the BP algorithm on the factor graph, $\mathcal{G}_{m,r_m}$, that is the Tanner graph of ${\mathcal{C}}_m^{(h)}$, augmented with additional \emph{extrinsic information} factor nodes, $\hat{f}_i: \{0,1\}\to \mathbb{R}$, for $i\in [n]$, and edges, $(x_i,\hat{f}_i)$, such that $\hat{f}_i$ acts on variable node $x_i$,
where if $\mathbf{b} = \mathbf{B}(i)$,
\[
\hat{f}_i(x_i) = \begin{cases}
	e^{+\beta\cdot \tilde{g}_{\mathbf{b}}\cdot(1\oplus x_i)},\ \text{if $\mathbf{b}\in \Gamma(g)$,}\\
	e^{+\beta\cdot \tilde{g}_{\mathbf{b}}\cdot x_i},\ \text{otherwise}.
\end{cases}
\]

\begin{figure}[h]
	\centering
	\resizebox{0.2\textwidth}{!}{
		
		


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
	
	%Shape: Square [id:dp8403288508079467] 
	\draw   (394,133.78) -- (419.22,133.78) -- (419.22,159) -- (394,159) -- cycle ;
	%Shape: Circle [id:dp41829979111166504] 
	\draw   (496.22,146.28) .. controls (496.22,138.83) and (502.26,132.78) .. (509.72,132.78) .. controls (517.17,132.78) and (523.22,138.83) .. (523.22,146.28) .. controls (523.22,153.74) and (517.17,159.78) .. (509.72,159.78) .. controls (502.26,159.78) and (496.22,153.74) .. (496.22,146.28) -- cycle ;
	%Straight Lines [id:da3928137029096386] 
	\draw    (419,146.78) -- (496.22,146.28) ;
	
	% Text Node
	\draw (400,139.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{i}$};
	% Text Node
	\draw (504,142.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{i}$};
	
	
\end{tikzpicture}
}
\caption{Extrinsic information factor nodes $f_i$ attached by an edge to variable node $x_i$, in the Tanner graph of $\mathcal{C}_m^{(h)}$.}
\label{fig:extrinsic}
\end{figure}

It can be verified that $e^{+\beta\cdot \tilde{\mathbf{g}}\cdot \tilde{\mathbf{h}}}\cdot\mathds{1}\{\mathbf{h}\in \mathcal{C}_m^{(h)}\} = \prod_{i\in [n]}\hat{f}_i(x_i)\cdot \prod_{a\in \mathcal{F}} f_a(x_{\partial a})$, where $f_a(\cdot)\in \mathcal{F}$ are the factors in the Tanner graph of $\mathcal{C}_m^{(h)}$, with $\prod_{a\in \mathcal{F}}f_a(x_{\partial a}) = \mathds{1}\{\mathbf{x}\in \mathcal{C}_m^{(h)}\}$. 
\begin{example}
Figure \ref{fig:factoreg} shows an example factor graph, $\mathcal{G}_{4,2}$, which is the Tanner graph of $\mathcal{C}_m^{(h)}$, augmented with the extrinsic information factor nodes, when $m=4$ and $r_m=2$. Note that the Tanner graph of $\mathcal{C}_m^{(h)}$ uses the parity-check matrix
\[
H = \begin{blockarray}{ccccccccc}
	& (0,0,0) & (0,0,1) & (0,1,0) & (0,1,1) & (1,0,0) & (1,0,1) & (1,1,0) & (1,1,1) \\
	\begin{block}{c[cccccccc]}
		x_3 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1\\
		x_2 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1\\
		x_1 & 0 & 0 & 0 & 0 & 1 & 1 & 1 & 1\\
		1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
	\end{block}
\end{blockarray},
\]
which is a generator matrix of the dual code, RM$(3,1)$, of $\mathcal{C}_m^{(h)}$. Note that the rows of $H$ correspond to the evaluations of the polynomials written on the left of the rows, which are of degree at most $1$, at the evaluation coordinates $\mathbf{x} = (x_1,x_2,x_3)$, which index the columns.
\end{example}

\begin{figure}[!t]
	\centering
	\resizebox{0.7\textwidth}{!}{
		

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,289); %set diagram left start at 0, and has height of 289
	
	%Shape: Ellipse [id:dp11867556334499563] 
	\draw   (278.22,111.89) .. controls (278.22,105.32) and (283.88,100) .. (290.86,100) .. controls (297.84,100) and (303.5,105.32) .. (303.5,111.89) .. controls (303.5,118.46) and (297.84,123.78) .. (290.86,123.78) .. controls (283.88,123.78) and (278.22,118.46) .. (278.22,111.89) -- cycle ;
	%Shape: Ellipse [id:dp8320396318228169] 
	\draw   (323.72,111.89) .. controls (323.72,105.32) and (329.38,100) .. (336.36,100) .. controls (343.34,100) and (349,105.32) .. (349,111.89) .. controls (349,118.46) and (343.34,123.78) .. (336.36,123.78) .. controls (329.38,123.78) and (323.72,118.46) .. (323.72,111.89) -- cycle ;
	%Shape: Ellipse [id:dp5690900409780586] 
	\draw   (369.22,111.89) .. controls (369.22,105.32) and (374.88,100) .. (381.86,100) .. controls (388.84,100) and (394.5,105.32) .. (394.5,111.89) .. controls (394.5,118.46) and (388.84,123.78) .. (381.86,123.78) .. controls (374.88,123.78) and (369.22,118.46) .. (369.22,111.89) -- cycle ;
	%Shape: Ellipse [id:dp24538071339195655] 
	\draw   (414.72,111.89) .. controls (414.72,105.32) and (420.38,100) .. (427.36,100) .. controls (434.34,100) and (440,105.32) .. (440,111.89) .. controls (440,118.46) and (434.34,123.78) .. (427.36,123.78) .. controls (420.38,123.78) and (414.72,118.46) .. (414.72,111.89) -- cycle ;
	%Shape: Ellipse [id:dp9165926883431132] 
	\draw   (460.22,111.89) .. controls (460.22,105.32) and (465.88,100) .. (472.86,100) .. controls (479.84,100) and (485.5,105.32) .. (485.5,111.89) .. controls (485.5,118.46) and (479.84,123.78) .. (472.86,123.78) .. controls (465.88,123.78) and (460.22,118.46) .. (460.22,111.89) -- cycle ;
	%Shape: Ellipse [id:dp6547258742549847] 
	\draw   (505.72,111.89) .. controls (505.72,105.32) and (511.38,100) .. (518.36,100) .. controls (525.34,100) and (531,105.32) .. (531,111.89) .. controls (531,118.46) and (525.34,123.78) .. (518.36,123.78) .. controls (511.38,123.78) and (505.72,118.46) .. (505.72,111.89) -- cycle ;
	%Shape: Ellipse [id:dp5298517344404583] 
	\draw   (551.22,111.89) .. controls (551.22,105.32) and (556.88,100) .. (563.86,100) .. controls (570.84,100) and (576.5,105.32) .. (576.5,111.89) .. controls (576.5,118.46) and (570.84,123.78) .. (563.86,123.78) .. controls (556.88,123.78) and (551.22,118.46) .. (551.22,111.89) -- cycle ;
	%Shape: Ellipse [id:dp12790715692740195] 
	\draw   (596.72,111.89) .. controls (596.72,105.32) and (602.38,100) .. (609.36,100) .. controls (616.34,100) and (622,105.32) .. (622,111.89) .. controls (622,118.46) and (616.34,123.78) .. (609.36,123.78) .. controls (602.38,123.78) and (596.72,118.46) .. (596.72,111.89) -- cycle ;
	%Shape: Square [id:dp0980936959631683] 
	\draw   (335,170.78) -- (360,170.78) -- (360,195.78) -- (335,195.78) -- cycle ;
	%Shape: Square [id:dp7478670727740837] 
	\draw   (395,170.78) -- (420,170.78) -- (420,195.78) -- (395,195.78) -- cycle ;
	%Shape: Square [id:dp0489506476039544] 
	\draw   (535,170.78) -- (560,170.78) -- (560,195.78) -- (535,195.78) -- cycle ;
	%Straight Lines [id:da588280016052462] 
	\draw    (336.36,123.78) -- (348,170.78) ;
	%Straight Lines [id:da17144386533080258] 
	\draw    (427.36,123.78) -- (348,170.78) ;
	%Straight Lines [id:da7237691849482373] 
	\draw    (518.36,123.78) -- (348,170.78) ;
	%Straight Lines [id:da5872899290519107] 
	\draw    (609.36,123.78) -- (348,170.78) ;
	%Straight Lines [id:da5950561796774235] 
	\draw    (381.86,123.78) -- (408,170.78) ;
	%Straight Lines [id:da37626928685601535] 
	\draw    (427.36,123.78) -- (408,170.78) ;
	%Straight Lines [id:da791700483632787] 
	\draw    (563.86,123.78) -- (408,170.78) ;
	%Straight Lines [id:da5554728543049094] 
	\draw    (609.36,123.78) -- (408,170.78) ;
	%Straight Lines [id:da8059636358806951] 
	\draw    (290.86,123.78) -- (550,169.78) ;
	%Straight Lines [id:da1920738522083043] 
	\draw    (336.36,123.78) -- (550,169.78) ;
	%Straight Lines [id:da9064133722799316] 
	\draw    (381.86,123.78) -- (550,169.78) ;
	%Straight Lines [id:da6859993620239205] 
	\draw    (427.36,123.78) -- (550,169.78) ;
	%Straight Lines [id:da5802321726106414] 
	\draw    (472.86,123.78) -- (550,169.78) ;
	%Straight Lines [id:da473576950845356] 
	\draw    (518.36,123.78) -- (550,169.78) ;
	%Straight Lines [id:da603480806128695] 
	\draw    (563.86,123.78) -- (550,169.78) ;
	%Straight Lines [id:da4039316279087375] 
	\draw    (609.36,123.78) -- (550,169.78) ;
	%Shape: Square [id:dp23729610814784974] 
	\draw   (280,53.78) -- (302,53.78) -- (302,75.78) -- (280,75.78) -- cycle ;
	%Shape: Square [id:dp06371456312715451] 
	\draw   (325,53.78) -- (347,53.78) -- (347,75.78) -- (325,75.78) -- cycle ;
	%Shape: Square [id:dp6635531962704774] 
	\draw   (371,53.78) -- (393,53.78) -- (393,75.78) -- (371,75.78) -- cycle ;
	%Shape: Square [id:dp2910414356748169] 
	\draw   (417,53.78) -- (439,53.78) -- (439,75.78) -- (417,75.78) -- cycle ;
	%Shape: Square [id:dp5127101339454895] 
	\draw   (461,53.78) -- (483,53.78) -- (483,75.78) -- (461,75.78) -- cycle ;
	%Shape: Square [id:dp6769266755594526] 
	\draw   (508,53.78) -- (530,53.78) -- (530,75.78) -- (508,75.78) -- cycle ;
	%Shape: Square [id:dp9488007017986179] 
	\draw   (553,53.78) -- (575,53.78) -- (575,75.78) -- (553,75.78) -- cycle ;
	%Shape: Square [id:dp5438497300919228] 
	\draw   (598,53.78) -- (620,53.78) -- (620,75.78) -- (598,75.78) -- cycle ;
	%Straight Lines [id:da8121181060049013] 
	\draw    (291,75.78) -- (290.86,100) ;
	%Straight Lines [id:da7375822997711297] 
	\draw    (336,75.78) -- (335.86,100) ;
	%Straight Lines [id:da5083050759722346] 
	\draw    (382,75.78) -- (381.86,100) ;
	%Straight Lines [id:da9740093216288499] 
	\draw    (428,75.78) -- (427.86,100) ;
	%Straight Lines [id:da6140512747767596] 
	\draw    (472,75.78) -- (471.86,100) ;
	%Straight Lines [id:da09893144162247025] 
	\draw    (519,75.78) -- (518.86,100) ;
	%Straight Lines [id:da6842934941393175] 
	\draw    (564,75.78) -- (563.86,100) ;
	%Straight Lines [id:da7966360480645057] 
	\draw    (609,75.78) -- (608.86,100) ;
	%Shape: Square [id:dp013396499490559877] 
	\draw   (465,170.78) -- (490,170.78) -- (490,195.78) -- (465,195.78) -- cycle ;
	%Straight Lines [id:da9267882602066787] 
	\draw    (518.36,123.78) -- (478,171.78) ;
	%Straight Lines [id:da731757422960738] 
	\draw    (472.86,123.78) -- (478,171.78) ;
	%Straight Lines [id:da11322724120965577] 
	\draw    (562.86,123.78) -- (478,171.78) ;
	%Straight Lines [id:da7215155788881816] 
	\draw    (609.36,123.78) -- (478,171.78) ;
	
	% Text Node
	\draw (285,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{1}$};
	% Text Node
	\draw (330,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{2}$};
	% Text Node
	\draw (375,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{3}$};
	% Text Node
	\draw (421,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{4}$};
	% Text Node
	\draw (466,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{5}$};
	% Text Node
	\draw (512,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{6}$};
	% Text Node
	\draw (558,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{7}$};
	% Text Node
	\draw (603,107.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 1; green, 35; blue, 78 }  ,opacity=1 ]  {$x_{8}$};
	% Text Node
	\draw (284,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{1}$};
	% Text Node
	\draw (329,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{2}$};
	% Text Node
	\draw (375,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{3}$};
	% Text Node
	\draw (420,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{4}$};
	% Text Node
	\draw (464,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{5}$};
	% Text Node
	\draw (512,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{6}$};
	% Text Node
	\draw (556,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{7}$};
	% Text Node
	\draw (601,57.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{f}_{8}$};
	% Text Node
	\draw (340,177.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{a}$};
	% Text Node
	\draw (400,177.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{b}$};
	% Text Node
	\draw (540,177.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{d}$};
	% Text Node
	\draw (470,177.18) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$f_{c}$};
	
	
\end{tikzpicture}
}
\caption{Factor graph $\mathcal{G}_{4,2}$ representing the product-form function $e^{+\beta\cdot \tilde{\mathbf{g}}\cdot \tilde{\mathbf{h}}}\cdot\mathds{1}\{\mathbf{h}\in \mathcal{C}_m^{(h)}\}$, when $m=4$ and $r_m=2$.}
\label{fig:factoreg}
\end{figure}

We run the BP algorithm on the factor graph $\mathcal{G}_{m,r_m}$, for large $m$ (we pick $m=13$) and large $\beta>0$ (we pick $\beta=40$)  (see equation \eqref{eq:statphy2}), for $100$ iterations each, for $200$ values of $\mathbf{g}$ picked uniformly at random from $\mathcal{C}_m^{(g)}$. We obtain that for all values of $\mathbf{g}$ chosen, the following are the BP fixed point messages, after suitable normalization, for $a\in \mathcal{F}$, which are the factor nodes of the Tanner graph.
\begin{align}
	\label{eq:fp1}
	\nu_{i\to a}^\star(0) = \begin{cases}
	\frac{e^\beta}{e^\beta+1},\quad \text{if $\mathbf{B}(i)\in \Gamma(g)$},\\
	\frac{e^{-\beta}}{e^{-\beta}+1},\quad \text{if $g(i)=1$},\\
	\frac{1}{2},\quad \text{otherwise},
	\end{cases}
\end{align}
with $\nu_{i\to a}^\star(1)  = 1-\nu_{i\to a}^\star(0)$, for $i\in [n]$ and $a\in \mathcal{F}$, and 
%\begin{align}
%	\nu_{i\to a}^\star(0) = \frac{e^\beta}{e^\beta+1},&\quad \nu_{i\to a}^\star(1) = \frac{1}{e^\beta+1},\quad \text{if $\mathbf{B}(i)\in \Gamma(g)$},\\
%	\nu_{i\to a}^\star(0) = \frac{e^{-\beta}}{e^{-\beta}+1},&\quad \nu_{i\to a}^\star(1) = \frac{1}{e^{-\beta}+1},\quad \text{if $g(i)=1$},\\
%	\nu_{i\to a}^\star(0) = \frac{1}{2},&\quad \nu_{i\to a}^\star(1) = \frac{1}{2},\quad \text{otherwise}.
%\end{align}
\begin{align}
	\label{eq:fp2}
	\hat{\nu}_{a\to i}^\star(0) = \frac12,
\end{align}
with $\hat{\nu}_{a\to i}^\star(1)  = 1-\hat{\nu}_{a\to i}^\star(0) = \frac12$, for all $i\in [n]$ and $a\in \mathcal{F}$.

We then compute $\hat{Z}_g^{\text{BP}}(\beta)$, using equations \eqref{eq:zbpstart}--\eqref{eq:zbpend}, and using the fixed point messages in \eqref{eq:fp1} and \eqref{eq:fp2} and obtain that for large enough $m$ and large enough $\beta$, 
\begin{equation}
		\label{eq:statphy3}
\log_2 \hat{Z}_g^{\text{BP}}(\beta)\geq (1-\delta_m)\cdot(2^{m-1}R+(\beta\log_2 e -1)\cdot\text{wt}(\tilde{\mathbf{g}})),
\end{equation}
where $\delta_m\xrightarrow{m\to \infty} 0$. Hence, by plugging \eqref{eq:statphy3} back into \eqref{eq:statphy2}, and using the fact that ${Z}_g^{\text{BP}}(\beta) = e^{-\beta \text{wt}(\tilde{\mathbf{g}})}\cdot \hat{Z}_g^{\text{BP}}(\beta)\cdot \mathds{1}\{\mathbf{g}\in \mathcal{C}_m^{(g)}\}$, we get that the BP approximation, $\mathsf{R}^{\text{BP},(1)}_{\hat{\mathcal{C}}}(R)$, of the rate $\mathsf{R}^{(1,\infty)}_{\hat{\mathcal{C}}}(R)$, obeys
\begin{align*}
	\mathsf{R}^{\text{BP},(1)}_{\hat{\mathcal{C}}}(R)&\geq  \limsup_{m\to \infty} \lim_{\beta \to \infty} \frac{\mathbb{E}_{\mathbf{g}\sim \text{Unif}\left(\hat{\mathcal{C}}_m^{g}\right)}\left[(1-\delta_m)\cdot(2^{m-1}R-\text{wt}(\tilde{\mathbf{g}}))\right]}{2^m}+\frac{R}{2}\\
	&= \limsup_{m\to \infty} \lim_{\beta \to \infty}  \frac{(1-\delta_m)R}{2} - \frac{\mathbb{E}_{\mathbf{g}\sim \text{Unif}\left(\hat{\mathcal{C}}_m^{g}\right)}\left[\text{wt}(\tilde{\mathbf{g}})\right]}{2^m}+\frac{R}{2}\\
	&= R - \frac38,
\end{align*}
%\begin{equation}
%	\label{eq:statphy3}
%\log_2 Z_g^{\text{BP}}(\beta)\geq (1-\delta)\cdot(2^{m-1}R-\text{wt}(\tilde{\mathbf{g}})),
%\end{equation}
%where $\delta\xrightarrow{m\to \infty} 0$. Hence, by plugging \eqref{eq:statphy3} back into \eqref{eq:statphy2}, we get that the BP estimate, $\mathsf{R}_{\hat{\mathcal{C}}}^{\text{BP}}(R)$, of the rate $\mathsf{R}^{(1,\infty)}_{\hat{\mathcal{C}}}(R)$, is at least $R-\lim_{m\to \infty} \frac{1}{2^m}\cdot\mathbb{E}_{\mathbf{g}\sim \text{Unif}\left(\hat{\mathcal{C}}_m^{g}\right)}[\text{wt}(\tilde{\mathbf{g}})]$,
where the last equality holds by Lemma \ref{lem:runcount}. We note that by Theorem \ref{thm:nonlin}, the BP approximation $\mathsf{R}^{\text{BP},(1)}_{\hat{\mathcal{C}}}(R)$ is a true lower bound on $\mathsf{R}^{(1,\infty)}_{\hat{\mathcal{C}}}(R)$. Although a direct computation of the BP approximation does not yield any more insight than the simple coding-theoretic arguments in the proof of Theorem \ref{thm:nonlin}, we note that it is indeed possible to improve this lower bound by loop calculus techniques \cite{chertkov, bashab,moriloop}. We set aside this question as future work.
